The Bayesian Infinitesimal Jackknife for Variance

The frequentist variability of Bayesian posterior expectations can provide meaningful measures of uncertainty even when models are misspecified. Classical methods to asymptotically approximate the frequentist covariance of Bayesian estimators such as the Laplace approximation and the nonparametric bootstrap can be practically inconvenient, since the Laplace approximation may require an intractable integral to compute the marginal log posterior, and the bootstrap requires computing the posterior for many different bootstrap datasets. We develop and explore the infinitesimal jackknife (IJ), an alternative method for computing asymptotic frequentist covariance of smooth functionals of exchangeable data, which is based on the "influence function" of robust statistics. We show that the influence function for posterior expectations has the form of a simple posterior covariance, and that the IJ covariance estimate is, in turn, easily computed from a single set of posterior samples. Under conditions similar to those required for a Bayesian central limit theorem to apply, we prove that the corresponding IJ covariance estimate is asymptotically equivalent to the Laplace approximation and the bootstrap. In the presence of nuisance parameters that may not obey a central limit theorem, we argue using a von Mises expansion that the IJ covariance is inconsistent, but can remain a good approximation to the limiting frequentist variance. We demonstrate the accuracy and computational benefits of the IJ covariance estimates with simulated and real-world experiments.

==> _high_dim_vm_detritus.tex <==
% I'm not sure yet whether I will want to keep any of this




% If we evaluate at $\t = 1$ so $\ftdist = \fdist$, then the posterior does not
% depend on the data, and the residual $\resid{T}(1)$ takes the form of a
% V--statistic, since
% %
% \begin{align*}
%     \htil[1](\x_n, \x_m) ={}&
%     \trace{
%     \left(\M(\fdist) + N \L(\fdist)\right)
%     \xbar_n \xbar_m^\trans 
%     }\\
%     \expect{\fdist(\x_n) \fdist(\x_m)}{\htil[1](\x_n, \x_m)} ={}& 0.
% \end{align*}
% %    
% Specifically, in the notation of \cite[Section
% 5.2.1]{serfling:1980:approximation}, $\resid{T}(1)$ is a V-statistic with
% (Serfling's) $m=2$, $\zeta_1 = 0$, and
% %
% \begin{align*}
%     \zeta_2 ={} \expect{\fdistnm}{\htil[1](\x_n, \x_m)^2}.
% \end{align*}
% %
% By Lemma A of the same section, the variance of the corresponding U-statistic is
% %
% %
% \begin{align*}
%     U :={}& \frac{1}{N(N-1)} \sumn \sum_{m\ne n}^N \htil[1](\x_n, \x_m)
%     &
%     \var{\fdist(\x_n) \fdist(\x_m)}{U} = 
%     \frac{2 \zeta_2}{N (N-1)}
% \end{align*}
% %

% Following \cite[Section 5.2.1]{serfling:1980:approximation}, the corresponding
% U-statistic satisfies











\hrulefill

\hrulefill

\hrulefill


% Then
% %
% \begin{align*}
% \expect{\fdist}{\sumn \ell(\x_n \vert \gamma, \lambda)} ={}& 
%     \frac{N}{G} \sumg \left( m_g (\log(\gamma) + \log(\lambda_g)) - \gamma \lambda_g\right) \\
% \postlf ={}&
% \textrm{Gamma}\left(\alpha + \frac{N}{G} m_g, \beta + \frac{N}{G} \gamma \right) \\
% \expect{\postlf}{\log \lambda_g} ={}& 
%     \mathrm{Digamma}\left(\alpha + \frac{N}{G} m_g\right) - \log\left(\beta + \frac{N}{G} \gamma \right) \\
% \var{\postlf}{\log \lambda_g} ={}& 
%     \mathrm{Trigamma}\left(\alpha + \frac{N}{G} m_g\right).
% \end{align*}
% %


% \todo{This is wrong --- since $\a_{ng}$ also multiplies the normalizing constant,
% it needs to be included in $\eta$.}
% For this model, and for $\ftdist = \fdist$,
% %
% \begin{align*}
% \eta(\gamma, \lambda) ={}& \log(\gamma) + \log(\lambda_g) \\
% \cov{\postlf}{\eta(\gamma, \lambda)} ={}& \diag{ \mathrm{Trigamma}\left(\alpha + \frac{N}{G} m\right) } \\
% \mu(\gamma) ={}& \log\left(\frac{\gamma}{\beta + \frac{N}{G} \gamma} \right) + \mathrm{Digamma}\left(\alpha + \frac{N}{G} m_g\right) \\
% \mubar(\gamma) ={}& 
%     \log\left(\frac{\gamma}{\beta + \frac{N}{G} \gamma} \right) -
%     \expect{\postgf}{\log\left(\frac{\gamma}{\beta + \frac{N}{G} \gamma} \right)}.
% % \ellunderbar(\x_n \vert \gamma, \lambda) ={}&
% %     \sumg (\y_n - m_g / G) \eta(\gamma, \lambda) \\
% % \ellbarbar(\x_n \vert \gamma, \lambda) ={}&
% %     \sumg (\y_n - m_g / G) \etabar(\gamma, \lambda).
% \end{align*}
% %

% Here, $\mubar(\gamma)$ is the same for all $g$, and $\cov{\postlf}{\eta(\gamma, \lambda)}$ does not depend on
% $\gamma$.  So $\L = 0$, and $\M$ is a $G \times G$ matrix with each entry equal to
% %
% \begin{align*}
%     \M_{11}(\fdist) = N^2 \expect{\postgf}{\gbar(\gamma) \mubar(\gamma) \mubar(\gamma)} = \ordlogp{1},
% \end{align*}
% %
% so
% %
% \begin{align*}
% \htil(\x_n, \x_m) ={}& \xbar_m^\trans \M(\fdist) \xbar_n = 
% \M(\fdist)_{11} \xbar_n^\trans \onevec \onevec^\trans \xbar_m^\trans
% \end{align*}

% Now, 

% %
% \begin{align*}
% \MoveEqLeft
% \expect{\fdist(\x_n)\fdist(\x_m)}{\htil(\x_n, \x_m)^2} 
% \\={}&
% \M(\fdist)_{11}^2
%     \expect{\fdist(\x_n)\fdist(\x_m)}{
%         \xbar_n^\trans \onevec \onevec^\trans \xbar_m 
%         \xbar_m^\trans \onevec \onevec^\trans \xbar_n}
% \\={}&
% \M(\fdist)_{11}^2
% \trace{
%     \expect{\fdist(\x_n)}{
%         \xbar_n \xbar_n^\trans
%     } 
%     \onevec \onevec^\trans
%     \expect{\fdist(\x_m)}{
%         \xbar_m \xbar_m^\trans
%     } 
%     \onevec \onevec^\trans
%     }
% \\={}&
% \M(\fdist)_{11}^2
% \trace{
%     \left( \frac{1}{G} \S - \frac{1}{G^2} m_g m_g^\trans\right)
%         \onevec \onevec^\trans
%     \left( \frac{1}{G} \S- \frac{1}{G^2} m_g m_g^\trans\right)
%         \onevec \onevec^\trans
%     }
% \\={}&
% \M(\fdist)_{11}^2 \left( 
%     \frac{1}{G^2} \trace{\S \onevec \onevec^\trans \S \onevec \onevec^\trans} -
%     \frac{2}{G^3} \trace{\S \onevec \onevec^\trans m_g m_g^\trans \onevec \onevec^\trans} +
%     \frac{1}{G^4} \trace{m_g m_g^\trans \onevec \onevec^\trans m_g m_g^\trans \onevec \onevec^\trans}
% \right)
% \\={}&
% \M(\fdist)_{11}^2 \left( 
%     \left(\frac{1}{G} \sumg v_g \right)^2 -
%     2 \left(\frac{1}{G} \sumg v_g \right) \left(\frac{1}{G} \sumg m_g \right)^2 +
%     \left(\frac{1}{G^4} \sumg m_g \right)^4
% \right).
% \end{align*}

% Here, because $\cov{\postlt}{\eta(\gamma, \lambda)}$ does not depend on $\gamma$ due to
% special problem structure, the residual actually vanishes.

% Furthermore, note that $\mu(\gamma)$ doesn't depend on the data, so it's not clear that
% the answer would be different if you took the correlation into account.



% \hrulefill

% \hrulefill

% \hrulefill


% Normal example.  Suppose that

% %
% \begin{align*}
% \ell(\y_n \vert \lambda_g, \gamma) ={}& -\frac{1}{2} \gamma^{-1} (\y_n - \lambda_g)^2 - \frac{1}{2} \log \gamma
%     \\={}& -\frac{1}{2} \gamma^{-1} \y_n^2 + \gamma^{-1} \lambda_g \y_n - 
%         \frac{1}{2} \gamma^{-1} \lambda_g^2 - \frac{1}{2} \log \gamma \\
% \expect{\fdist(\y_n \vert \a_{ng}=1)}{\ell(\y_n \vert \lambda, \gamma)} ={}& 
%     -\frac{1}{2} \gamma^{-1} \meang \v_g + \gamma^{-1} \meang \lambda_g \m_g - 
%         \frac{1}{2} \gamma^{-1} \meang \lambda_g^2 - \frac{1}{2} \log \gamma \\
% \postlf ={}& \normdist\left( \lambda_g \vert m_g , \frac{G}{N} \gamma \right)
% \end{align*}
% %

% This will have an annoying extra term, but will have a covariance that depends on $\gamma$.




% \hrulefill

% \hrulefill

% \hrulefill














%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Proof of \lemref{resid_form}.}\applabel{resid_form_proof}
\begin{proof}[]
    %
    Under \exref{grouped_exp}, 
    %
    \begin{align*}
    \expect{\ftdist(\x_n)}{\z_n} ={} \frac{m}{G}
    \quad\quad\textrm{and}\quad\quad
    \zbar_n = \z_n - \frac{m}{G}
    \quad\quad\textrm{and}\quad\quad
    \expect{\ftdist(\x_n)}{\z_n \z_n^\trans} ={}
        \frac{\S}{G} - \frac{m m^\trans}{G^2}
    \end{align*}
    %
    and
    %
    \begin{align*}
        \expect{\postglt}{\eta(\gl)} 
        % = \expect{\postgt}{\eta(\gl)} + \mu(\gamma) - \mu(\gamma) 
        = \expect{\postgt}{\mu(\gamma)}.
    % \cov{\ftdist}{\x_n \x_n^\trans} ={}& \frac{1}{G} \S - \frac{1}{G^2} m m^\trans.
    \end{align*}
    %
    So
    %
    \begin{align*}
        \ellbarbar(\x_n \vert \gamma, \lambda) = 
        \zbar_n^\trans \etabar(\gamma, \lambda) =
        \left(\z_n - m / G\right)^\trans \left( 
            \eta(\gl) - \mu(\gamma) + \mubar(\gamma)
        \right).
    \end{align*}
    %
    We can then write (c.f.~\eqref{highdim-resid})
    %
    \begin{align*}
    \htil(\x_n, \x_m) ={}&
    N^2 \expect{\postglt}{
        \gbar(\gamma)
        \ellbarbar(\x_n \vert \gl)
        \ellbarbar(\x_m \vert \gl)    
        }
    \\={}&
    N^2 \expect{\postglt}{
        \gbar(\gamma)
        \left( \zbar_n^\trans \etabar(\gamma, \lambda) \right)
        \left( \zbar_m^\trans \etabar(\gamma, \lambda) \right)
    }
    \\={}&
    N^2 \zbar_m^\trans
    \expect{\postglt}{
        \gbar(\gamma)
        \etabar(\gamma, \lambda)
        \etabar(\gamma, \lambda)^\trans 
    } \zbar_n 
    .
    % N^2 \trace{\expect{\postglt}{
    %     \gbar(\gamma)
    %     \etabar(\gamma, \lambda)
    %     \etabar(\gamma, \lambda)^\trans 
    % } \zbar_n \zbar_m^\trans 
    % }.
    \end{align*}
    
    The inner expectation can be expanded as
    %
    \begin{align*}
    \MoveEqLeft
    \expect{\postglt}{
        \gbar(\gamma)
        \etabar(\gamma, \lambda)
        \etabar(\gamma, \lambda)^\trans 
    } 
    ={} \\&
    \expect{\postgt}{
        \gbar(\gamma)
        \expect{\postlt}{
            \left(\eta(\gamma, \lambda) - \mu(\gamma) + \mubar(\gamma) \right)
            \left(\eta(\gamma, \lambda) - \mu(\gamma) + \mubar(\gamma) \right)^\trans
        }
    } 
    ={} \\&
    \expect{\postgt}{
        \gbar(\gamma)
        \left( 
        \expect{\postlt}{
            \left(\eta(\gamma, \lambda) - \mu(\gamma)\right)
                \left(\eta(\gamma, \lambda) - \mu(\gamma)\right)^\trans
        }  + 
        \mubar(\gamma) \mubar(\gamma)^\trans
        \right)}
    ={} \\&
    \expect{\postgt}{
        \gbar(\gamma)
        \left( 
        \cov{\postlt}{\eta(\gamma, \lambda)} + 
        \mubar(\gamma) \mubar(\gamma)^\trans
        \right)}
    ={} \\&
    N^{-1} \L + N^{-2} \M,
    \end{align*}
    %
    by \defref{high_dim_exp_terms}.  The result follows by combining expressions.
    %
\end{proof}
    
    

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of \lemref{grouped_exp}.}\applabel{grouped_exp_proof}


So the limiting behavior is determined by

\begin{align*}
\MoveEqLeft
\expect{\fdist(\x_n) \fdist(\x_m)}{\htil[1](\x_n, \x_m)^2} 
\\={}& 
\expect{\fdist(\x_n) \fdist(\x_m)}{
    \trace{
    \left(\M(\fdist) + N \L(\fdist)\right)
    \xbar_n \xbar_n^\trans   
    \left(\M(\fdist) + N \L(\fdist)\right)
    \xbar_m \xbar_m^\trans   
    }
}
\\={}&
\trace{
    \left(\M(\fdist) + N \L(\fdist)\right)
    \left(\frac{1}{G} \S - \frac{1}{G^2} m m^\trans\right)
    \left(\M(\fdist) + N \L(\fdist)\right)
    \left(\frac{1}{G} \S - \frac{1}{G^2} m m^\trans\right)
}
\\={}&
\frac{1}{G^2} \trace{\M \S \M \S} +
\frac{1}{G^3} \trace{\M \S \M m m^\trans} +
\frac{N}{G^2} \trace{\M \S \L \S} +
\frac{1}{G^3} \trace{\M \S \L m m^\trans} +
\\{}&
\frac{1}{G^3} \trace{\M m m^\trans \M \S} +
\frac{1}{G^4} \trace{\M m m^\trans \M m m^\trans} +
\frac{N}{G^3} \trace{\M m m^\trans \L \S} +
\frac{N}{G^4} \trace{\M m m^\trans \L m m^\trans} +
\\{}&
\frac{N}{G^2} \trace{\L \S \M \S} +
\frac{N}{G^3} \trace{\L \S \M m m^\trans} +
\frac{N^2}{G^2} \trace{\L \S \L \S} +
\frac{N^2}{G^3} \trace{\L \S \L m m^\trans} +
\\{}&
\frac{N}{G^3} \trace{\L m m^\trans \M \S} +
\frac{N}{G^4} \trace{\L m m^\trans \M m m^\trans} +
\frac{N^2}{G^3} \trace{\L m m^\trans \L \S} +
\frac{N^2}{G^4} \trace{\L m m^\trans \L m m^\trans}.
\end{align*}
%
where we write $\L = \L(\fdist)$ and $\M = \M(\fdist)$ for compactness.


  For example,

%
\begin{align*}
\frac{1}{G^2} \trace{\M(\fdist) \S \M(\fdist) \S}  = 
\frac{1}{G^2} \trace{\S^{1/2} \M(\fdist) \S^{1/2} \S^{1/2} \M(\fdist) \S^{1/2}}  \le 
\frac{1}{G^2} \sqrt{\Sigma(\M) \Sigma(\M)} = \ordlog{1}.
\end{align*}
%

Similarly,

%
\begin{align*}
\frac{1}{G^3} \trace{\M(\fdist) \S \M(\fdist) m m^\trans} ={}&
\frac{1}{G^3} m^\trans \S^{-\dagger/2} \S^{1/2}\M(\fdist) \S^{1/2} \S^{1/2} \M(\fdist) 
    \S^{1/2} \S^{-\dagger/2}m 
\\\le{}& 
\frac{1}{G^3} \norm{\S^{-\dagger/2} m}_2^2 \sigma_G(\S^{1/2}\M(\fdist) \S^{1/2})^2
= \ordlog{1}.
\end{align*}
%
In summary,
%
\begin{itemize}
\item It takes a factor of $1/G$ to kill a factor of $\M$,
\item It takes a factor of $1/\sqrt{G}$ to kill a factor of $\L$,
\item It takes a factor of $1/G$ to kill a factor of $m m^\trans$,
\item And the $\S$ can always be assimilated into these bounds.
\end{itemize}
%


Applying these rules, we get
\begin{align*}
\expect{\fdist(\x_n) \fdist(\x_m)}{\htil[1](\x_n, \x_m)^2} 
\le{}&
\ordlog{1} +
\ordlog{1} +
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{1}{\sqrt{G}}} +
\\{}&
\ordlog{1} +
\ordlog{1} +
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{N}{\sqrt{G}}} +
\\{}&
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{N^2}{G}} +
\ordlog{\frac{N^2}{G}} +
\\{}&
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{N}{\sqrt{G}}} +
\ordlog{\frac{N^2}{G}} +
\ordlog{\frac{N^2}{G}} 
\\={}&
    \ordlog{1} +
    \ordlog{\frac{N}{\sqrt{G}}} +
    \ordlog{\frac{N^2}{G}}.
\end{align*}
%
Under the assumption that $G / N \rightarrow \alpha \in (0, \infty)$, this
gives
%
\begin{align*}
    \expect{\fdist(\x_n) \fdist(\x_m)}{\htil[1](\x_n, \x_m)^2} = \ordlog{N}
\end{align*}
%
It follows that
%
\begin{align*}
\expect{\fdistnm}{\left( \frac{1}{N^2} \sum_{n \ne m} \sqrt{N} \htil[1](\x_n, \x_m) \right)^2} 
    ={}&
\frac{N}{N^4} 
\expect{\fdist(\x_n) \fdist(\x_m)}{
        \sum_{n \ne m} \sum_{n' \ne m'} 
        \htil[1](\x_n, \x_m) 
        \htil[1](\x_{n'}, \x_{m'})
} 
\\={}&
\frac{2 N (N - 1)}{N^3} 
\expect{\fdist(\x_n) \fdist(\x_m)}{
        \htil[1](\x_n, \x_m)^2
}
\\={}& \ord{N^{-1}} \ordlogp{N} = \ordlogp{1}.
\end{align*}
%
In the second to last equation, we use the fact that $\expect{\fdist(\x_n) \fdist(\x_m)}{
    \htil[1](\x_n, \x_m) 
    \htil[1](\x_{n'}, \x_{m'})
} = 0$ unless $n=n'$ and $m=m'$ or $n=m'$ and $m=m'$, of which there are
$2 N (N - 1)$ such terms.





==> appendices/delta_method_standard_errors.tex <==

In order to evaluate our results we need to estimate standard errors for each of
these quantities.  Note that, even in the absence of MCMC error (e.g. as $M
\rightarrow \infty$), we would not expect $\gcovijhat = \gcovboothat$, as the two
numerically distinct despite being consistent estimates of the same quantity.
Similarly, under correct specification, we do not expect $\gcovijhat = \gcovboothat =
\gcovbayes$ even when there is no MCMC error.  Thus, when comparing our
estimated $\gcovijhat$, $\gcovboothat$, and $\gcovbayeshat$, it is important to
consider sampling error due to the randomness in the original sample $\xvec$ in
addition to MCMC error.

To do so, we rely on two algorithms to estimate the frequentist and MCMC
variability of scalar covaraince estimates.  We will apply these two algorithms
to the components of $\gcovijhat$ and $\gcovboothat$, neglecting sampling
covariance between elements of the matrices.  Of course, the elements of
the covaraince matrices are not independent, and so the standard errors we
compute are useful heuristics but should not be used for formal hypothesis
testing.

Our first algorithm uses the classical delta method for the sampling covariance
of a sample covariance of IID draws.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[H]
\caption{Delta Method for IID Data}\algrlabel{deltamethodalg}
\textbf{Inputs (global variables):}\\
$a = (a_1, \ldots, a_N)$ \Comment{Scalar IID draws}\\
$b = (b_1, \ldots, b_N)$ \Comment{Scalar IID draws}\\
%
\begin{algorithmic}
%\algrlabel{Compute Sampling covariance of}
%
\Function{SampleCov}{$\alpha$, $\beta$}
\State \Return
    $\meann \alpha_n \beta_n - \meann \alpha_n \meann \beta_n$
\EndFunction\\
%
%\Call{SampleCov}{$a$, $b$}
\Function{SampleCovDeltaMethodSE}{$a$, $b$}
    \State $\bar{a} \gets \meann a_n$
    \State $\bar{b} \gets \meann b_n$
    \State $\bar{ab} \gets \meann a_n b_n$
    \State $ab \gets \meann a \odot b$
    \Comment{The $\odot$ operator denotes the element-wise product}
    \State $\nabla h \gets \left(1, -\bar{a}, -\bar{b}\right)$
    \State $S \gets
    \left[
    \begin{matrix}
    \Call{SampleCov}{ab, ab} &
    \Call{SampleCov}{ab, a} &
    \Call{SampleCov}{ab, b} \\
    \Call{SampleCov}{a, ab} &
    \Call{SampleCov}{a, a} &
    \Call{SampleCov}{a, b} \\
    \Call{SampleCov}{b, ab} &
    \Call{SampleCov}{b, a} &
    \Call{SampleCov}{b, b} \\
    \end{matrix}
    \right]$
    \State \Return $\sqrt{\frac{1}{N} \nabla h^T S \nabla h}$
\EndFunction\\
%
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The bootstrap draws of the posterior mean, $\gamma^*_b$, are IID given the
original dataset, $\xvec$, since the MCMC chains and bootstrap samples are
independent across $b$. The variability in the draws $\gamma^*_b$ reflect both
MCMC and sampling variability, since both the MCMC chains and bootstrap draws
are different for each.  Consequently, we can estimate both the frequentist and
MCMC variability in $\gcovboothat$ by applying \algrref{deltamethodalg} to each
pair of components of $\gamma^*_b$.  Let $\gamma^*_{i\cdot}$ denote the
length-$B$ vector of the $i$-the element of the posterior means, and let
$\seboot$ be the $\gdim\times\gdim$ matrix whose $i,j$-th element is
%
\begin{align*}
%
\seboot_{ij} :=
    \Call{SampleCovDeltaMethodSE}{\gamma^*_{i\cdot}, \gamma^*_{j\cdot}}.
%
\end{align*}
%
We can thus approximately expect that
$\gcovboothat_{ij} \in \left(\gcovtrue_{ij} \pm 2 \seboot_{ij} \right)$.

Similarly, we can treat the $\infl_n$ of \algrref{ijalg} as IID draws from
$\fdist(\x_n)$, and use \algrref{deltamethodalg} to estimate the frequentist
sampling error of the $i,j$-the component $\gcovij_{ij}$.  Specifically,
letting $\infl_{i\cdot}$ denote the length-$N$ vector containing the $i$-th
component of the influence score, we define
%
\begin{align*}
%
\seijfreq_{ij} :=
    \Call{SampleCovDeltaMethodSE}{\infl_{i\cdot}, \infl_{j\cdot}}.
%
\end{align*}
%
We can thus approximately expect that
$\gcovij_{ij} \in \left(\gcovtrue_{ij} \pm 2 \seijfreq_{ij} \right)$.

However, we cannot use \algrref{deltamethodalg} to capture the difference
between $\gcovij$ and $\gcovijhat$.  To do so, we block bootstrap the MCMC chain
with a block size much larger than the estimated effective sample size,
applying \algrref{ijalg} to each resampled chain, computing an estimated
MCMC standard error, $\seijmcmc$.  Finally, we combine the two sources of
error assuming independence, giving, for each $i,j$,
%
\begin{align*}
%
\seij_{ij} := \sqrt{(\seijmcmc_{ij})^2 + (\seijfreq_{ij})^2}.
%
\end{align*}
%
We can thus approximately expect that
$\gcovijhat_{ij} \in \left(\gcovtrue_{ij} \pm 2 \seij_{ij} \right)$.

% Note that
% multivariate autoregressive techniques such as \cite{flegal:2020:mcmcse}
% will be difficult to employ...


==> detritus.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Details from the intuition section, probably not necessary.

Recall from
\eqref{ij_terms} that $\infl_n = \cov{\post}{\theta, \ell(\x_n \vert \theta)}$.
By the BCLT, $\expect{\post}{\theta} = \thetahat + O_p(N^{-1})$ and
$\expect{\post}{\ell(\x_n \vert \theta)} = \ell(\x_n \vert \thetahat) +
O_p(N^{-1})$, so that
%
\begin{align*}
%
N^{-1} \infl_n = \cov{\post}{\theta, \ell(\x_n \vert \theta)} =
\expect{\post}{(\theta - \thetahat) (\ell(\x_n \vert \theta) - \ell(\x_n
\vert \thetahat)} + O_p(N^{-2}).
%
\end{align*}
%
We can Taylor expand $\ell(\x_n \vert \theta)$ around $\thetahat$ inside the
preceding expectation and substitute for $\tau = \sqrt{N}(\theta - \thetahat)$,
giving
%
\begin{align*}
%
\MoveEqLeft
(\theta - \thetahat)
    (\ell(\x_n \vert \theta) - \ell(\x_n \vert \thetahat)) =
N^{-1} \tau \tau^T \ellgrad{1}(\x_n \vert \thetahat) +
N^{-3/2} O(\norm{\tau}_2^3).
%
\end{align*}
%
Again by the BCLT, $\expect{\post}{\tau \tau ^T} = \infohat^{-1} + O_p(N^{-1})$,
and $\expect{\post}{\norm{\tau}_2^3}$ is bounded with probability approaching
one. Combining these facts gives
%
\begin{align*}
\infl(\x_n)
    ={}& N \cov{\post}{\theta, \ell(\x_n \vert \theta)}
    &\quad\textrm{(\eqref{ij_terms})} \nonumber\\
={}&
    N \expect{\post}{
        (\theta - \thetahat)
        (\ell(\x_n \vert \theta) - \ell(\x_n \vert \thetahat)} + O_p(N^{-2})
&\quad\textrm{(BCLT)} \nonumber\\
={}&
    \expect{\post}{\tau \tau^T}
    \ellgrad{1}(\x_n \vert \thetahat) + O_p(N^{-3/2})
&\quad\textrm{(Taylor series)} \nonumber\\
={}&
    \infohat^{-1} \ellgrad{1}(\x_n \vert \thetahat) + O_p(N^{-1}).
&\quad\textrm{(BCLT)} 
\end{align*}
%







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The high dim posteriors don't conincide


\subsubsection{$\postg$ and $\postgf$ do not coincide as $N \rightarrow \infty$}

We first show that, in the case of \exref{re}, the difference between
expectations with respect to $\postg$ and $\postgf$ does not vanish, even as $N
\rightarrow \infty$. Though we discuss the specific case of \exref{re} in detail
because we can actually compute the limiting behavior of both $\postg$ and
$\postgf$, the root cause of the problem can be seen to be general, which is
that data expectations do not commute with log marginalization over $\lambda$.
However, we show that as the conditional posterior $\postl$ concentrates, the
difficulty vanishes.

%
\begin{ex}\exlabel{re_fdist}
%


In the case of \exref{re}, the posterior $\postgf$ is determined by the
expectation $\expect{\fdist(\xn)}{\ell(\xn \vert \gamma, \lambda)}$, which can
be re-arranged to give
%
\begin{align*}
%
% \MoveEqLeft
\postgf \propto{}&
% \int \exp\left(N
% \expect{\fdist(\xn)}{\ell(\xn \vert \gamma, \lambda)}
%  \right) \prior(\lambda \vert \gamma) d\lambda \, \prior(\gamma)
% %
% \\={}&
\exp\left( G \mathscr{L}_{\fdist}(\gamma) \right) \prior(\gamma)
\textrm{ where}
\\
% \int \exp\left(
% N \sumg \expect{\fdist(\a_{0g})}{\a_{0g}}
%     \expect{\fdist(\y_0 \vert \a_{0g} = 1)}
%     {\ell(\y_0 \vert \gamma, \lambda_g, \a_{0g} = 1)}
%  \right) \prodg \prior(\lambda_g) d\lambda_g \prior(\gamma)
% =\\{}&
% \exp\left(G  \meang \log \int \exp\left(
%     \frac{N}{G} \expect{\fdist(\y_0 \vert \a_{0g} = 1)}
%     {\ell(\y_0 \vert \gamma, \lambda_g, \a_{0g} = 1)}
% \right) \prior(\lambda_g) d \lambda_g \right) \prior(\gamma).
\likf(\gamma) :={}&
    \meang \log \int \exp\left(
        \frac{N}{G} \expect{\fdist(\y_0 \vert \a_{0g} = 1)}
        {\ell(\y_0 \vert \gamma, \lambda_g, \a_{0g} = 1)}
    \right) \prior(\lambda_g) d \lambda_g.
%
\end{align*}
%
Comparing $\likf(\gamma)$ with the true limiting distribution $\lik(\gamma)$
given \exref{re_conc}, we see that, in general, the functions $\likf(\gamma)$
and $\lik(\gamma)$ are meaningfully different, even when $G, N \rightarrow
\infty$.  In particular, we expect $\argsup_{\gamma} \lik(\gamma) \ne
\argsup_{\gamma} \likf(\gamma)$, because expectation does not commute with the
random effect marginalization.

% For the von Mises expansion, this implies that, when $\T(\gdist) =
% \expect{\p(\gl \vert \gdist, N)}{\phi(\gamma)}$, $\T(\fndist) - \T(\fdist)$ does
% not vanish as $N \rightarrow \infty$, even though the posterior $\postg$ does
% concentrate.  In general, we thus expect the residual $\resid{T}(\t)$ to
% fail to vanish as well.
%
\end{ex}

In the nested random effect case of \exref{re} we can confirm directly that
$\lim_{N \rightarrow \infty} \T(\fndist) \ne \T(\fdist)$ and $\lim_{N
\rightarrow \infty} \infl_n \ne \infltil_n$, and so the IJ covariance can be
expected to be inconsistent, even were the residual to vanish (which it does not ---
see \secref{high_dim_residual} below).

In essence, the failure in \exref{re_fdist} of $\postg$ to coincide with
$\postgf$ is because the limiting behavior of $\postg$ is determined by
marginalizing over the random effects and then taking a data expectation,
whereas $\postgf$ first takes a data expectation, and then marginalizes over the
random effects.  That is, in a stylized form,
%
\begin{align}\eqlabel{expect_marg_commute}
%
% \expect{\fdist(\xn)}{\log
% \int \exp(f(\xn, \lambda)) \postl d\lambda} \ne
% \log \int \exp\left(\expect{\fdist(\xn)}{f(\xn, \lambda)}
% \postl d \lambda \right).
\expect{\fdist(\xn)}{
    \log \expect{\p(\lambda)}{\exp(f(\xn, \lambda))}
    }
\ne
\log \expect{\p(\lambda)}{
    \exp\left(
        \expect{\fdist(\xn)}{f(\xn, \lambda)}
        \right)
}.
%
\end{align}
%
Thus, because $\lambda$-marginalization and expectations do not commute, we
expect the failure of $\postg$ and $\postgf$ to asymptotically coincide to be
general.

However, the difference between the left and right hand sides of
\eqref{expect_marg_commute} disappears when the conditional posterior $\postl$
is concentrated.  In particular, in the stylized form of
\eqref{expect_marg_commute}, if $\expect{\p(\lambda)}{f(\lambda)} \approx
f(\hat{\lambda})$, then the exponential and log cancel, and the inequality
becomes an (approximate) equality. Heuristically, this suggests that, though
$\abs{\infltil_n - \infl_n}$ may not go to zero when the dispersion of $\postl$
does not vanish, the difference may be practically small when the spread of
$\postl$ is practically small.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% old high-dim stuff




It is
difficult, and beside our present purpose, to state useful general conditions
for global--local models under which $\postg$ concentrates.  Instead, in
\assuref{conc} below, we simply assume the features of
\thmref{bayes_clt_main,bayes_clt_vm} we needed to analyze the von Mises
expansions without assuming how they arise.

\begin{assu}\assulabel{conc} Assume that the posterior $\postgt$ ``concentrates''
    in the sense $\gammahat(t) \plim \gammatrue$ for some $\gammatrue$
    uniformly in $\t \in [0, 1]$, and that
    sufficiently regular expectations of the form
    $\expect{\postg}{\phi(\gamma)}$, $\expect{\postg}{\phi(\gamma, \x_n)}$, and
    $\expect{\postg}{\phi(\gamma, \x_n, \x_m)}$ admit expansions
    analogous to those of \thmref{bayes_clt_main,bayes_clt_vm}. Furthermore, we
    assume without further elaboration that all the posterior expectations we
    consider are ``sufficiently regular'' in this sense.  (See \assuref{conc} of
    \appref{von_mises_details} for a precise statement.)
\end{assu}

In general,  we expect \assuref{conc} to hold if
there exists a smooth function $\lik(\gamma)$, analogous to $\lik(\theta)$ of
\defref{loglik_def}, such that
%
%\begin{align*}
%
$\int \postgl d \lambda =
\postg \propto \exp\left(N \lik(\gamma)\right)$
approximately, for large $N$.
%
%\end{align*}
%
\Assuref{conc} is satisfied by posteriors such as those of \exref{re}, to which
we can apply \thmref{bayes_clt_main,bayes_clt_vm} after marginalizing (see
\exref{re_conc} in \appref{von_mises_details} for more details). Beyond this,
the imprecision of \assuref{conc} is not a major liability, since we will use it
to preclude the possibility of a result like \thmref{finite_dim_resid} for
global--local models.

Using \assuref{conc}, we can use the Tower property to write the terms of
\lemref{expansion_terms} in terms of expectations over $\postg$ that we
can analyze.  In particular,
%
\begin{align*}
%
% \expect{\postf}{\gbar(\gamma) \ellbarbar(\x_n \vert \gl)} ={}&
\infltil_n ={}&
N \expect{\postgf}{
    \gbar(\gamma) \expect{\postlf}{\ellbarbar(\x_n \vert \gl)} } 
\quad\textrm{and}\quad \\
\htil(\x_n, \x_m)
% \expect{\postft}{
%         \gbar(\gamma)
%         \ellbarbar(\x_n \vert \gl)
%         \ellbarbar(\x_m \vert \gl)
%         } 
={}&
N^2 \expect{\postgt}{
    \gbar(\gamma)
    \expect{\postlt}{
        \ellbarbar(\x_n \vert \gl)
        \ellbarbar(\x_m \vert \gl)    
    }
}.
\end{align*}
%
In contrast to the finite--dimensional case, we see that the log likelihood
terms have been replaced by their marginal expectation over $\postlt$.  


The conditional expectations will determine the behavior of the von--Mises expansion, and so
we give them their own symbols.

\begin{defn}\deflabel{ceterms}
%
Define the quantities
%
\begin{align*}
%
\ceone[\gdist](\x_n \vert \gamma) :={}
    \expect{\p(\lambda | \gdist, N, \gamma)}{\ellbarbar(\x_n \vert \gl)}
\quad\textrm{and}\quad
\cetwo[\gdist](\x_n, \x_m \vert \gamma) :={}
    \expect{\p(\lambda \vert \gdist, N, \gamma)}{
        \ellbarbar(\x_n \vert \gl)
        \ellbarbar(\x_m \vert \gl)
    }.
%
\end{align*}
%
We now show that the under-- and over--bars respect \defref{centering}.

By Fubini's theorem, $\expect{\fdist(\xn)}{\ceone(\xn \vert \gamma)} = 0$ and
$\expect{\fdist(\x_n)\fdist(\x_m)}{\cetwo(\x_n, \x_m \vert \gamma, \t)} = 0$.
Similarly, the gradients satisfy $\expect{\fdist(\xn)}{\ceonegrad{k}(\xn \vert
\gamma)} = 0$ and $\expect{\fdist(\x_n)\fdist(\x_m)}{\cetwograd{k}(\x_n, \x_m
\vert \gamma, \t)} = 0$.

The posterior centering gives $\expect{\postgt}{\ceone(\x_n \vert \gamma)} = 0$
by the Tower property.  But, in general, $\expect{\postgt}{\cetwo(\x_n, \x_m
\vert \gamma)} \ne 0$.  Since the posterior centering is not a function of
$\gamma$ (see \defref{centering}), in general the derivatives
$\expect{\postgt}{\ceonegrad{k}(\x_n \vert \gamma)} \ne  0$ for $k \ge 1$, so we
write them without an overbar.
%
\end{defn}

\begin{assu}\assulabel{high_dim} Let \assuref{conc} hold, and let
$\thetaball{\delta}$ denote a neighborhood of $\gammatrue$.  Assume further that
the expectations $\expect{\fdist(\xn)}{\ceonegrad{1}(\x_n \vert \gamma)^2}$ and
$\expect{\fdist(\x_n) \fdist(\x_m)}{\cetwograd{k}(\x_n, \x_m \vert \gamma)^2}$,
for $k \in \{1,2\}$, are all uniformly finite and bounded away from zero for
$\gamma \in \thetaball{\delta}$ and all sufficiently large $N$.
%
\end{assu}


%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{thm}\thmlabel{highdimresid}(See proof in \appref{high_dim_resid}.)
%
Let \assuref{high_dim} hold.  Then
%
\begin{itemize}
\item $\frac{1}{\sqrt{N}} \sumn \infltil_n \dlim \normdist\left(0, V \right)$,
where $\gcovij \plim V$.  (TODO: you need uniform integrability)
\item $\sqrt{N} \resid{\t} = 
    \ordp{N^{1/2} \sqrt{
        \expect{\fdist(\x_n) \fdist(\x_m)}{\cetwograd{1}(\x_n, \x_m \vert \gammahat(\t))^2}
    }}
    \plim \infty$ for all $\t \in [0,1]$.
\end{itemize}
%
It follows that, in general, the IJ covariance estimate is inconsistent.
%
\end{thm}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Old, less general exponential family example

We have $\ell(\x_n \vert \gamma, \lambda) = \sumg \y_n \a_{ng} \gamma \lambda_g - A(\gamma, \lambda)$,
%
which we can rewrite as
\begin{align*}
    \ell(\x_n \vert \gamma, \lambda) = \y_n \a_n^\trans \lambda \gamma
    \quad\textrm{where}\quad
    \a_n = (\a_{n1}, \ldots, \a_{nG})^\trans
    \quad\textrm{and}\quad
    \lambda = (\lambda_{1}, \ldots, \lambda_{G})^\trans.
\end{align*}
%
Define $m_g := \expect{\fdist(\y_n | \a_{ng} = 1)}{\y_n}$, 
$v_g := \var{\fdist(\y_n | \a_{ng} = 1)}{\y_n}$, 
$\mu_g(\gamma) := \expect{\postlt}{\lambda_g}$, and let
%
\begin{align*}
    m := (m_1, \ldots, m_G )^\trans
    \quad\textrm{and}\quad
    v := \diag{v_1, \ldots, v_G}
    \quad\textrm{and}\quad
    \mu := (\mu_1, \ldots, \mu_G )^\trans.
\end{align*}
%
Further, define 
\begin{align*}
    \eta := \lambda \gamma
        \quad\textrm{and}\quad
    \alpha(\gamma) := \gamma \mu(\gamma).
\end{align*}
%
Then we can write
%
\begin{align*}
    \ellbarbar(\x_n \vert \gamma, \lambda) = \left(\y_n \a_n - m / G \right)^\trans \etabar.
\end{align*}
%
Then
%
\begin{align*}
\V ={}& \expect{\fdist(\xn)}{
    \ellbarbar(\xn \vert \gamma, \lambda) \ellbarbar(\xn \vert \gammatil, \lambdatil)
}
\\={}& \trace{\etabar \etabar^\trans 
    \expect{\fdist(\xn)}{ \left(\y_n \a_n - m / G \right) 
                          \left(\y_n \a_n - m / G \right)^\trans}}
\\={}& G^{-1} \trace{\etabar \etabar^\trans \left(v + m m^\trans / G \right)} < \infty.
\end{align*}

We now compute $\rv(\gamma, \gammatil)$.  First,
%
\begin{align*}
\etabar = 
    \gamma \lambda - \expect{\postgt}{\gamma \expect{\postlt}{\lambda}} = 
    % \gamma (\lambda - \mu(\gamma)) + \gamma \mu(\gamma)- \expect{\postgt}{\gamma \mu(\gamma)}
    \gamma (\lambda - \mu(\gamma)) + \alphabar(\gamma).
\end{align*}
%
Then $\expect{\postlt}{\lambda - \mu(\gamma)} = 0$, so
%
\begin{align*}
\expect{\postlt}{\etabar \etabar^\trans}
    ={}& \Lambda(\gamma) + \alphabar(\gamma) \alphabar(\gamma)^\trans,
    \quad\textrm{where}\quad \Lambda(\gamma) := \cov{\postlt}{\lambda} \textrm{ is diagonal.}
\end{align*}
%
So
%
\begin{align*}
\rv(\gamma, \gammatil) ={}& 
    G^{-2} \trace{\left(\Lambda(\gamma) + 
                        \alphabar(\gamma) \alphabar(\gamma)^\trans \right) 
                  \left(v + 
                        m m^\trans / G \right)
                  \left(\Lambda(\gammatil)  + 
                        \alphabar(\gammatil) \alphabar(\gammatil)^\trans \right)
                  \left(v + 
                        m m^\trans / G \right)
    }. 
% \\=& G^{-2} \trace{\Lambda(\gamma) v \Lambda(\gammatil) v} +             % 0000
% \\& G^{-3} \trace{\Lambda(\gamma) v \Lambda(\gammatil) m m^\trans} +     % 0001
% \\& G^{-2} \trace{\Lambda(\gamma) v \alphabar(\gammatil) \alphabar(\gammatil)^\trans v} +  % 0010
% \\& G^{-2} \trace{\Lambda(\gamma) v \alphabar(\gammatil) \alphabar(\gammatil)^\trans m m^\trans} + % 0011
% %
% \\& G^{-3} \trace{\Lambda(\gamma) m m^\trans \Lambda(\gammatil) v} +   % 0100
% \\& G^{-4} \trace{\Lambda(\gamma) m m^\trans \Lambda(\gammatil) m m^\trans} +     % 0101
% \\& G^{-3} \trace{\Lambda(\gamma) m m^\trans \alphabar(\gammatil) \alphabar(\gammatil)^\trans v} +  % 0110
% \\& G^{-4} \trace{\Lambda(\gamma) m m^\trans \alphabar(\gammatil) \alphabar(\gammatil)^\trans m m^\trans} + % 0111
% %
% \\& G^{-2} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans v \Lambda(\gammatil) v} +             % 1000
% \\& G^{-3} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans v \Lambda(\gammatil) m m^\trans} +     % 1001
% \\& G^{-2} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans v \alphabar(\gammatil) \alphabar(\gammatil)^\trans v} +  % 1010
% \\& G^{-2} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans v \alphabar(\gammatil) \alphabar(\gammatil)^\trans m m^\trans} + % 1011
% %
% \\& G^{-3} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans m m^\trans \Lambda(\gammatil) v} +   % 1100
% \\& G^{-4} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans m m^\trans \Lambda(\gammatil) m m^\trans} +     % 1101
% \\& G^{-3} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans m m^\trans \alphabar(\gammatil) \alphabar(\gammatil)^\trans v} +  % 1110
% \\& G^{-4} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans m m^\trans \alphabar(\gammatil) \alphabar(\gammatil)^\trans m m^\trans}  % 1111
%
\end{align*}
%
The product inside the trace can be expanded to $2^4 = 16$ terms, each including one each of:
%
\begin{itemize}
\item Either the diagonal $\Lambda(\gamma)$ or outer product $\alphabar(\gamma) \alphabar(\gamma)^\trans$;
\item Either the diagonal $v$ or the outer product $m m^\trans / G$;
\item Either the diagonal $\Lambda(\gammatil)$ or outer product $\alphabar(\gammatil) \alphabar(\gammatil)^\trans$;
\item Either the diagonal $v$ or the outer product $m m^\trans / G$.
\end{itemize}
%
Rather than analyze each of the 16 terms separately, we can observe some patterns.  First,
let's look at the behavior of the two extremes, where we include either all
diagonal terms or all outer product terms.  First, 
%
\begin{align*}
    G^{-2} \trace{\Lambda(\gamma) v \Lambda(\gammatil) v} =
    G^{-1} \sumg \Lambda_{gg}(\gamma) \Lambda_{gg}(\gammatil) v_g^2
\end{align*}
%
is $G^{-1}$ times a function of the form $f(\gamma, \gammatil)$, since the trace
gives a sum of $G$ products of the $\Lambda(\cdot)$ diagonals.  Next,
%
\begin{align*}
G^{-4} \trace{\alphabar(\gamma) \alphabar(\gamma)^\trans m m^\trans \alphabar(\gammatil) \alphabar(\gammatil)^\trans m m^\trans} 
    ={}&
G^{-4} (m^\trans \alphabar(\gamma))^2 
       (m^\trans \alphabar(\gammatil))^2
\end{align*}
%
will be a product of four sums, each over $G$ entries, where each summand
contains either an entry of $\alphabar(\gamma)$ or $\alphabar(\gammatil)$. The
result will be an sum of $G^4$ terms, each of the form
$\alphabar_{i}(\gamma) \alphabar_{j}(\gamma) \alphabar_{k}(\gammatil) \alphabar_{l}(\gammatil)$,
a product of two each posterior--centered functions of $\gamma$ and $\gammatil$.
Since the $G^{4}$ cancels with the $G^4$, the result is an $O(1)$
sum of products of two each posterior--centered functions of $\gamma$
and $\gammatil$.

From these two calculations, some patterns emerge:
%
\begin{itemize}
    \item Even when including only diagonal terms, the trace adds an order
          of $G$ to the final expression.
    \item Including a $v$ term does not change the order of the final expression.
    \item Including a $m m^\trans / G$ term adds an additional order of $G$ in the trace, but
          adds a factor of $1/G$, and so does not change the order of the final
          expression.
\end{itemize}
%
Consequently, the order of the final expression does not depend on whether
we include a $v$ or a $m m^\trans / G$ term.  Next,
%
\begin{itemize}
    \item Including a diagonal $\Lambda(\gamma)$ term does not change the order
          of the trace, but introduces a non--centered term depending
          on $\gamma$, and
    \item Including a $\alphabar(\gamma) \alphabar(\gamma)^\trans$
          term both adds an order of $G$ in the trace, and introduces two 
          posterior--centered functions of $\gamma$.
\end{itemize}
%
Now, by \assuref{high_dim} \itemref{highdim_conc},
%
\begin{align*}
    \expect{\postgt}{\gbar(\gamma) \Lambda_g(\gamma)} = 
    \expect{\postgt}{\gbar(\gamma) \overline{\Lambda}_g(\gamma)} = 
    \ordp{N^{-1}}
    \quad\textrm{and}\quad
    \expect{\postgt}{\gbar(\gamma) \alphabar_{i}(\gamma) \alphabar_{j}(\gamma)} = 
        \ordp{N^{-2}},
\end{align*}
%
so, putting everything together, and using the fact that $G = O(N)$,
%
\begin{align*}
\expect{\postgt}{\expect{\postgtilt}{
    \gbar(\gamma)  \gbar(\gammatil)  
    \rv(\gamma, \gammatil)
}} 
={}& \ordp{G^{-1} N^{-1} N^{-1}}  +& 
    \textrm{Including } \Lambda(\gamma) \textrm{ and } \Lambda(\gammatil) \\
{}& \ordp{N^{-1} N^{-2}}  +& 
    \textrm{Including } \alphabar(\gamma) \alphabar(\gamma)^\trans \textrm{ and } \Lambda(\gammatil) \\
{}& \ordp{G N^{-2} N^{-2}}  & 
    \textrm{Including } \alphabar(\gamma) \alphabar(\gamma)^\trans 
        \textrm{ and } \alphabar(\gamma) \alphabar(\gamma)^\trans \\
={}& \ordp{N^{-3}}.
\end{align*}
%
So 
%
\begin{align*}
    \expect{\fdist(\x_n)\fdist(\x_m)}{
        \htil(\x_n, \x_m)^2
    } = 
    N^4  \expect{\postgt}{\expect{\postgtilt}{
        \gbar(\gamma)  \gbar(\gammatil)  
        \rv(\gamma, \gammatil)
    }} 
    = \ordp{N^{-1}}.
\end{align*}
%












% Currently mostly stuff taken from the main text that we don't want to delete




% \subsection{Higher dimension discussion}


% We now turn to studying the von Mises expansion for high-dimensional
% global--local models.  Let us briefly recap.  Recall that we turned to von Mises
% expansions because, even when the marginal posterior of the global parameter
% $\postg \propto \exp(N \likhat(\gamma))$ for some $\likhat(\gamma)$ converging
% to a deterministic $\lik(\gamma)$, the sampling behavior of $\likhat(\gamma)$
% under $\fdist$ may be complicated, since it may no longer be a sum of IID
% contributions after marginalization over $\lambda$.  For this reason, the
% approach of \thmref{ij_consistent} cannot be applied.  As an alternative, we can
% form a von Mises expansion, an approach which we showed in
% \thmref{finite_dim_resid} is also capable of proving consistency of the IJ
% covariances in the finite-dimensional case.  The advantage of the von Mises
% expansion is that it can be applied to high-dimensional settings since it does
% not make explicit use of the sampling behavior of $\likhat(\gamma)$.  As in
% \secref{von_mises}, the relevant quantities will all be posterior expectations
% under $\postg$ which, again, can be studied using
% \thmref{bayes_clt_main,bayes_clt_vm}.

% Two key results characterized our proof of consistency in finite dimensions:
% %
% \begin{enumerate}
% %
% \item The posteriors $\postf$ and $\post$ coincide asymptotically, so that
% $\infl_n \approx \infltil_n$ and so $\covhat{n \in [N]}{\infl_n} \plim
% \cov{\fdist{\infltil_0}}{\infltil_0}$.
% % \begin{itemize}
% %     \item[$\Rightarrow$]  $\T(\fndist) - \T(\fdist) \plim 0$ and
% %     $\sqrt{N}\abs{\infltil_n - \infl_n} \plim 0$.
% % \end{itemize}
% %
% \item The residual $\sqrt{N} \resid{T}(\t) \plim 0$ uniformly in $\t$, so that
% $\sqrt{N}(\T(\fndist) - \T(\fdist))$ is the same as $\frac{1}{\sqrt{N}} \sumn
% \infltil_n$ asymptotically.
% %
% \end{enumerate}

% However, we will find that neither of these two results obtain in
% high-dimensional global--local models, even when the marginal posterior $\postg$
% is asymptotically concentrated.  Specifically, in high dimensions, in general:
% %
% \begin{enumerate}
% %
% \item $\postgf$ does not coincide with $\postg$ , even as $N \rightarrow
% \infty$, so that $\infl_n$ and $\infltil_n$ converge to different constants,
% as do $\expect{\postgf}{\g(\gamma)}$ and $\expect{\postg}{\g(\gamma)}$.
% %
% \item The residual $\sqrt{N} \resid{T}(\t)$ does not vanish as $N \rightarrow
% \infty$, so that $\sqrt{N}(\T(\fndist) - \T(\fdist))$ is not the same as
% $\frac{1}{\sqrt{N}} \sumn \infltil_n$, even asymptotically.
% %
% \end{enumerate}
% %
% Of course, these two failure modes are related via \eqref{t_expansion_highdim}.
% If $\T(\fndist) - \T(\fdist)$ does not vanish as $N \rightarrow \infty$, the
% difference must be accounted for either in the influence scores or in the
% residual, typically in both.\footnote{It is possible to form functionals in
% general for which $\T(\fndist) - \T(\gdist)$ fails to vanish even when the
% residual vanishes for some $\gdist$.  Consider, for example, a linear functional
% $\T(\gdist) = \int x \gdist(d x)$ and a von Mises expansion around some
% distribution not equal to the true data-generating distribution.  However,
% outside of such specially constructed cases, one would typically expect the
% residual term to account at least in part for asymptotic bias in $\T(\fndist) -
% \T(\fdist)$.}

% Although these results are negative, we also argue heuristically that, when the
% conditional posterior $\postl$ is itself not too dispersed, then the von Mises
% expansion holds approximately. We essentially argue that, even in asymptotic
% regimes where the spread of $\postl$ does not go to zero and the IJ is
% inconsistent, the IJ covariance will remain a useful if formally inconsistent
% estimate, particularly given its computational simplicity.














% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{A von Mises expansion}

% We will begin by defining the terms in a von Mises expansion for global--local
% models. Analogously to \secref{von_mises}, let us define $\T(\gdist) :=
% \expect{\p(\gl \vert \gdist, N)}{\g(\gamma)}$, the difference from
% \eqref{expectation_functional} being that we have restricted $\g(\theta)$ to
% depend only on the ``global'' parameters $\gamma$. As before, $\T(\fndist) =
% \expect{\postgl}{\g(\gamma)} = \expect{\postg}{\g(\gamma)}$, and we can form the
% series expansions as \eqref{t_expansion}, giving
% %
% \begin{align}
% %
% \T(\fndist) - \T(\fdist) ={}& \meann \infltil_n + \resid{T}(\ttil)
%     \quad\textrm{where} \eqlabel{t_expansion_highdim}
% \\
% \infltil_n :={}& \cov{\postgf}{\g(\gamma), \ell(\x_n \vert \gamma, \lambda)}
%     = \expect{\postgf}{\gbar(\gamma) \ellbarbar(\x_n \vert \gamma, \lambda)}
% \nonumber \\
% \resid{T}(\t) ={}&
%     \frac{1}{2}
%     \meannm
%     N^2 \expect{\postglt}{
%         \gbar(\gamma)
%         \ellbarbar(\x_n \vert \gamma, \lambda)
%         \ellbarbar(\x_m \vert \gamma, \lambda)}. \nonumber
% %
% \end{align}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% High dim discussion




% As in the finite-dimensional case, we see that the influence score takes the
% form of $N$ times a posterior covariance. When $\postg$ concentrates as in
% \assuref{conc}, by the same reasoning as in the proof of \thmref{ij_consistent},
% for a typical datapoint $\x_n$,
% %
% \begin{align*}
% %
% \infl_n = \A{2}  \gbargrad{1}(\gammahat) \ceonegrad{1}(\x_n \vert \gammahat) +
% \ordp{N^{-1}} = \ordp{1}.
% %
% \end{align*}
% %
% Thus, the influence scores of a typical datapoint do not diverge as $N
% \rightarrow \infty$.\footnote{As in the finite-dimensional case, the extremal
% influence scores may of course diverge.}  If we additionally assume that the
% entries of $\ceonegrad{1}(\xn \vert \gammatrue)$ are square integrable under
% $\fdist(\xn)$, then we expect $N^{-1/2} \sumn \infl_n$ to obey a FCLT as well.
% Of course, as show in the previous section, we expect that $\abs{\infl_n -
% \infltil_n}$ does not go to zero, since $\infl_n$ are evaluated at $\fndist$ and
% $\infltil_n$ are evaluated at $\fdist$, and $\postg$ and $\postgf$ do not, in
% general, concentrate at the same location asymptotically.

% While the influence score is governed by $\ceone(\x_n \vert \gamma)$, the
% residual is governed by $\cetwo(\x_n, \x_m \vert \gamma)$.  Marginally,
% $\expect{\postgt}{\cetwo(\x_n, \x_m \vert \gamma)} \ne 0$ is a posterior
% covariance involving $\lambda$, and does not, in general, go to zero.
% Correspondingly, $\cetwo(\x_n, \x_m \vert \gammahat(\t))$ also does not go to
% zero.  Similarly, the derivatives $\cetwograd{k}(\x_n, \x_m \vert
% \gammahat(\t))$ do not, in general, go to zero.  In fact, $\cetwo(\x_n, \x_m
% \vert \gammahat)$ is asymptotically equivalent to a covariance with respect to
% $\postlt$, since we can write
% %
% \begin{align*}
% %
% \ellbarbar(\x_n \vert \gl) ={}&
% \ellunderbar(\x_n \vert \gl) -
%     \expect{\postglt}{\ellunderbar(\x_n \vert \gl)} +
% \\&
% \expect{\postlt}{\ellunderbar(\x_n \vert \gl)} -
%     \expect{\postlt}{\ellunderbar(\x_n \vert \gl)}.
% %
% \end{align*}
% %
% By \assuref{conc},
% %
% \begin{align*}
% %
% \expect{\p(\lambda | \ftdist, N, \gammahat(\t))}
%        {\ellunderbar(\x_n \vert \gammahat(\t), \lambda)} -
% \expect{\postglt}{\ellunderbar(\x_n \vert \gl)} = \ordp{N^{-1}},
% %
% \end{align*}
% %
% so
% %
% \begin{align}\eqlabel{cetwoiscov}
% %
% \cetwo(\x_n, \x_m \vert \gammahat(\t)) ={}&
% \cov{\p(\lambda \vert \fdist, N, \gammahat(\t))}
%     {\ellunderbar(\x_n \vert \gammahat(\t), \lambda),
%      \ellunderbar(\x_m \vert \gammahat(\t), \lambda)} + \ordp{N^{-1}}.
% %
% \end{align}

% Thus,  under our assumption that $\postlt$ does not concentrate, we expect
% $\cetwo(\x_n, \x_m \vert \gamma)$ and its derivatives to be non-degenerate
% random variables.  In particular, we expect that, for $k \ge 0$, the variance
% %
% \begin{align*}
% %
% \var{\fdistnm}{\cetwograd{k}(\x_n, \x_m \vert \gamma)} \ne 0.
% %
% \end{align*}
% %
% In this case, we expect $\sqrt{N} \resid{\t}$ to diverge, as we now state
% formally.



% Recall that $\sqrt{N} \resid{\t} = \meannm \sqrt{N} \htil(\x_n, \x_m)$ where $\htil(\x_n,
% \x_m) = N^2 \expect{\postgt}{\gbar(\gamma) \cetwo(\x_n, \x_m \vert \gamma,
% \t)}$. Using \assuref{conc}, $\expect{\postgt}{\gbar(\gamma) \cetwo(\x_n, \x_m
% \vert \gamma, \t)}$ can be expressed as $\ordp{N^{-1}}$ times derivatives of
% $\cetwo(\x_n, \x_m \vert \gamma, \t)$ evaluated at $\gammahat(\t)$.  Asymptotic
% concentration of V-statistics of the form given by our $\htil(\x_n, \x_m)$
% contribute another factor of order $N^{-1}$ (see \cite[Chapter
% 5]{serfling:1980:approximation}, with the key result summarized in
% \appref{vstats}).  But since $\var{\fdistnm}{\cetwograd{1}(\x_n, \x_m \vert
% \gamma, \t)}$ remains bounded away from zero, a factor of $N^{1/2}$ remains.
% %
% % End proof sketch


% In \appref{high_dim_resid} we include a more detailed analysis showing that, for
% our working \exref{re}, we expect $\var{\fdistnm}{\cetwograd{1}(\x_n, \x_m \vert
% \gamma)}$ to remain bounded away from zero, no matter how large $G$
% is.  In fact, when $G \gg N$ in \exref{re}, each observation will belong
% to only one group with arbitrarily high probability, and yet $\sqrt{N}
% \resid{\t}$ does not vanish.  This shows that the failure of the von-Mises
% expansion in high dimensions is not due only to the possibility of repeated
% groups under sampling from $\fdist$.

% When the local posterior $\postlt$ is approximately concentrated --- i.e., its
% covariances are small if not vanishing --- then by the decomposition
% \eqref{cetwoiscov} we expect the residual to be practically small.  Indeed, if
% $\var{\fdistnm}{\cetwograd{1}(\x_n, \x_m \vert \gamma)} = \ord{N^{-1}}$, as it
% would be if $\postlt$ obeyed \assuref{conc}, then one can see by the proof sketch
% of \thmref{highdimresid} that we would have $\sqrt{N} \resid{\t} \plim 0$, as
% expected.









% % We showed above that $\gcovij$ is consistent under the  conditions of
% % \thmref{bayes_clt_main} as long as $\sup_{\t \in [0, 1]} \sqrt{N} \resid{T}(\t)
% % \plim 0$, so that is all that remains to be shown.

% % As in the proof of \thmref{ij_consistent}, we write $\gbar(\theta)
% % \ellbarbar(\x_n \vert \theta) \ellbarbar(\x_m \vert \theta)$ as a product of
% % terms centered at $\thetahat$. We then apply
% % \thmref{bayes_clt_main,bayes_clt_vm} to each resulting term, showing that each
% % is of order $N^{-2}$.  As a consequence, $\htil(\x_n, \x_m \vert \t)$ can be
% % written as a sum of products of derivatives of $\gbar(\theta)$ and
% % $\ellbarbar(\x_n \vert \theta)$, all evaluated at $\thetahat(\t)$, times
% % $\sqrt{N}$, plus a square summable residual that vanishes asymptotically.

% % Next we use the fact that $\sup_{\t \in [0,1]} \thetahat(\t) \plim \thetatrue$
% % to show that, with probability approaching one, each non-vanishing contribution
% % to $\htil(\x_n, \x_m \vert \t)$ is bounded in probability by a quantity of the
% % form
% % %
% % \begin{align*}
% % %
% % \sup_{\theta \in \thetaball{\delta}} \norm{
% % \meann \ellunderbargrad{k}(\x_n \vert \theta)}_2 \plim 0,
% % %
% % \end{align*}
% % %
% % where convergence to zero follows from
% % $\expect{\fdist(\x_n)}{\ellunderbargrad{i}(\x_n \vert \thetahat)} = 0$ by the
% % interchange of expectation with respect to $\fdist(\x_n)$ and differentiation
% % with respect to $\theta$, together with \lemref{ulln}.
% % %
% \end{proofsketch}
    




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Step three: Evaluate the residual $\resid{T}(\t)$}


% %%%% ....


% We see that $\resid{T}(\t)$ takes the form of a V-statistic, so named precisely
% because of its occurrence in von Mises expansions (\cite[Chapter
% 5]{serfling:1980:approximation}). Note that, for fixed $\ftdist$,
% $\expect{\fdist(\x_n)}{\expect{\fdist(\x_m)}{\htil(x_n, x_m \vert \t)}} = 0$. We
% can thus study $\htil(x_n, x_m \vert \t)$ in order to establish conditions under
% which $\sup_{\t \in [0,1]} \sqrt{N} \resid{\T}(\t) \plim 0$, in which case the
% IJ covariance is consistent.  Conversely, in conditions when the above
% V-statistic does not vanish, we expect the IJ covariance to be inconsistent in
% general.

% The quantity $\htil(x_n, x_m \vert \t)$ is a posterior expectation of a product
% of three quantities which are centered with respect to the integrating posterior
% $\postft$.  In general, we expect expectations of three centered quantities to
% converge to zero faster than to, i.e., faster than a covariance, a fact which we
% will prove using the following variant of \thmref{bayes_clt_main}.

% % Using \thmref{bayes_clt_vm}, we are show in \thmref{finite_dim_resid} below that
% % $\gcovij$ is consistent without explicit reference to the known sandwich
% % covariance form of the limiting variance.  The keys to the proof will be
% % the facts that:
% % %
% % \begin{itemize}
% % %
% % \item Posterior quantities converge to their expectation at rate $N^{-1}$
% % (\thmref{bayes_clt_main}),
% % \item Posterior covariances converge at $N^{-1}$ (\thmref{bayes_clt_main}),
% % \item Posterior expectations of products of three centered quantities
% % converge at rate $N^{-2}$ (\thmref{bayes_clt_vm}),
% % \item Asymptotically, both $\post$ and $\postf$ concentrate
% % at the same point (\lemref{bclt_okay_t}).
% % %
% % \end{itemize}
% % %

% With \thmref{bayes_clt_vm}, we are now in a position to state formal conditions
% under which the von Mises expansion is able to reproduce the direct proof of the
% consistency of $\gcovij$ in \thmref{ij_consistent}.





% Informally, we note that the summands in the first-order term given in
% \eqref{term1} are closely related to our influence scores, since
% %
% \begin{align*}
%     %
%     \expect{\postf}{\gbar(\theta)\ellbarbar(\x_n \vert \theta)} ={}&
%     \cov{\postf}{\g(\theta), \ellunderbar(\x_n \vert \theta)} := \frac{\infltil_n}{N}.
% %
% \end{align*}
% %
% This $\infltil_n$ involves covariance with respect to $\postf$ instead of $\postfn$,
% and uses the centered $\ellunderbar(\x_n \vert \theta)$ in place of $\ell(\x_n
% \vert \theta)$, but is otherwise equal to our influence scores $\infl_n$. 
% The randomness in $\infltil_n$ is due to the $\x_n$ term alone, unlike
% $\infl_n$, in which the posterior itself is also random. Since
% $\expect{\fdist(\x_n)}{\infltil_n} = \ordlogp{N^{-1}}$ by
% \thmref{bayes_clt_main}, we have, by the ordinary frequentist CLT,
% % \footnote{Note that $\expect{\fdist(\x_n)}{\infl_n} \ne 0$ in
% % general due to the $\x_n$ dependence in the posterior.  Since $\thetahat -
% % \thetatrue = \ordp{N^{-1/2}}$ in general, $\infl_n - \infltil_n =
% % \ordp{N^{-1/2}}$ as well, so $\expect{\fdist(\x_n)}{\infl_n}$ cannot be
% % neglected when considering the limiting distribution of $N^{-1/2} \sumn
% % \infl_n$.  It is for this reason that it is more convenient to form the Taylor
% % series expansion around $\t=0$ and $\fdist$ than around $\t=1$ and $\fndist$.
% % }
% \begin{align*}
%     %
%     \frac{1}{\sqrt{N}} \sumn \infltil_n
%         \dlim \normdist\left(0, \lim_{N\rightarrow \infty}
%             \cov{\fdist(\xn)}{\infltil_0} \right).
%     %
% % \quad\textrm{where}\quad
% % \cov{\fdist(\xn)}{\infltil_0} \plim \gcovtrue.
% \end{align*}
% %
% In our finite--dimensional IID setting, we expect $\cov{\fdist(\xn)}{\infltil_0}
% \plim \gcovtrue$, and so for the IJ covariance to be consistent.  In
% high--dimensional settings, we will show that $\frac{1}{\sqrt{N}} \sumn
% \infltil_n$ still typically converges to a non--degenerate random variable whose
% variance is consistently estimated by the IJ covariance, but that the residual
% also fails to vanish.


==> experiments_singular.tex <==

In the previous example, the IJ was not strictly necessary because we could
compute $\thetahat$ in closed form.  In this section, we present a simple
simulated example where $\thetahat$ cannot be easily computed, and yet the IJ
still provides useful results.  The key feature of the model that renders the IJ
useful is that finding $\thetahat$ requires performing a complicated
integral to marginalize out latent parameters.  When $\theta$ comprises some
subset of the parameters, the rest having been marginalized out, then it
is plausible that $\thetahat$ optimizes an objective function that is
approximately quadratic near its optimum, but which is difficult to evaluate
because of the necessary marginalization.  One could turn to MCMC
to find the posterior, and the IJ covariance to estimate the frequentist
covariance of the posterior mean.

To illustrate the problem consider the following simple random effects model
with responses, $y_n \in \mathbb{R}$, regressors $r_n \in \mathbb{R}$, and group
indicator vectors $z_n \in \{0, 1\}^K$, for $n=1,\ldots,N$.  We assume that all
three are conditionally IID, so $\x_n = (y_n, r_n, z_n)$. Define the regression
parameter $\beta \in \mathbb{R}$, random effect vector $\mu \in \mathbb{R}^K$,
and variances $\sigma_y^2$ and $\sigma_\mu^2$.  We will not specify priors
precisely as we will shortly be using the default diffuse priors provided by
\texttt{rstanarm}; let us take the priors as given and independent. Then we can
model
%
\begin{align}\eqlabel{simple_sim_model}
%
y_n | z_n, r_n, \beta, \mu, \sigma_y^2 \indep&
    \normdist(\cdot | \beta r_n + z_n^T \mu, \sigma_y^2) \nonumber\\
\mu_k | \sigma_\mu \indep&
    \normdist(\cdot | 0, \sigma_\mu^2).
%
\end{align}

How good is the MAP estimate for this model?  The answer depends on which
variables are marginalized out of the posterior.  Suppose, for example, we
optimize over all the parameters:
%
\begin{align*}
%
\hat\beta, \hat\sigma_y, \hat\sigma_\mu, \hat\mu :=
    \argmax \ell(\xvec | \beta, \sigma_y, \sigma_\mu, \mu) +
            \ell(\mu | \sigma_\mu) +
            \ell(\beta) + \ell(\sigma_y) + \ell(\sigma_\mu).
%
\end{align*}
%
Since we are computing $\hat\mu$, optimizing over all parameters including the
random effects is prone to under-estimate the variance $\sigma_y$, particularly
when $K$ is large relative to $N$.  (This phenomenon is the substance of the
Neyman-Scott paradox \cite{freedman:2005:neymanscott}.)  For this reason, one
does not typically optimize over $\mu$ for such a model.  Rather, one optimizes
the marginal posterior (or an approximation thereof):
%
\begin{align}\eqlabel{singular_map}
%
\hat\beta, \hat\sigma_y, \hat\sigma_\mu :=
    \argmax & \log \int p(\xvec | \beta, \sigma_y, \sigma_\mu, \mu)
        p(\mu | \sigma_\mu) d\mu  +
        %\nonumber\\
       \ell(\beta) + \ell(\sigma_y) + \ell(\sigma_\mu)
      \nonumber\\
= \argmax & \sumn \ell(\x_n | \beta, \sigma_y, \sigma_\mu) +
\ell(\beta) + \ell(\sigma_y) + \ell(\sigma_\mu).
%
\end{align}
%
For Gaussian models such as this one, the integral can be computed in closed
form. In the general case, methods such as marginal maximum likelihood
estimation (MMLE) approximate the integral, e.g., with a Laplace approximation.

However, it is possible to generate data $\xvec$ so that the MAP of
\eqref{singular_map} estimates $\hat\sigma_\mu = 0$ for sufficiently
non-informative priors.  In particular, $\hat\sigma_\mu = 0$ can occur if the
responses $y_n$ have sufficiently low covariance with the indicators $z_n$ after
accounting for the regressors $r_n$.  Such degenerate covariance estimates are
more common in real datasets with multiple random effects, though even a single
random effect is enough.  When $\hat\sigma_\mu = 0$, the second derivative
of the log posterior is degenerate at the optimum, and classical methods
for approximating frequentist variances cannot be directly applied.

To deal with the degenerate variance estimate, one might additionally integrate
out the variance parameters $\sigma_\mu$ and $\sigma_y$ and form the MAP over
the regression parameters alone,
%
\begin{align}\eqlabel{nonsingular_map}
%
\hat\beta :=
    \argmax & \log \int p(\xvec | \beta, \sigma_y, \sigma_\mu, \mu)
        p(\mu | \sigma_\mu) p(\sigma_\mu) p(\sigma_y)
        d\mu d \sigma_\mu d\sigma_y + \ell(\beta)
        \nonumber\\
= \argmax & \sumn \ell(\x_n | \beta) + \ell(\beta).
%
\end{align}
%
Unlike \eqref{singular_map}, the integral over \eqref{nonsingular_map} is not
likely to be well-approximated by a Laplace approximation for the same reasons
that the \eqref{singular_map} provides a poor approximation to the overall
posterior.  Indeed, it is precisely to approximate integrals of the sort found
in \eqref{nonsingular_map} that one typically turns to MCMC.  It may well be the
case that the behavior of $\hat\beta$, as given by \eqref{nonsingular_map}, is
approximately normal.  However, since MCMC is required to evaluate the
objective function, \eqref{nonsingular_map} is not typically used.  Rather,
one would simply run MCMC on the entire problem, $\beta$ included.

In short, if we take $g(\theta) = \theta := \beta$ in this problem, then
\eqref{nonsingular_map} gives us reason to believe that $\thetahat \approx
\expect{\post}{\theta}$ and that both are approximately normally distributed,
due to the concentration of the marginal log likelihood $\sumn \ell(\x_n |
\theta)$.  However, we cannot easily compute the objective function or its
derivatives, since $\ell(\x_n | \theta)$ involves an intractable integral.
Nevertheless, we can run MCMC on all the parameters and use the IJ to
approximate the frequentist variance of the limiting distribution of
$\expect{\post}{\theta}$.  It is in precisely such cases that the IJ covariance
is most useful.

As a demonstration, we draw data from the following misspecified data generating
process.  Fix $K = \simNumRe$ and $N = \simNumObs$.  For each $n=1,\ldots,N$
we draw independently
%
\begin{align}\eqlabel{simple_sim_dgp}
%
r_n \iid \normdist(\cdot | 0, 1)
\quad\quad\quad
\epsilon_n \iid \normdist(\cdot | 0, 1)
\quad\quad\quad
y_n := r_n + r_n^2 \epsilon_n.
%
\end{align}
%
Under the generating process of \eqref{simple_sim_dgp}, simple numerical
simulation shows that the MMLE package \texttt{lme4} results in a numerically
singular fit ($\hat\sigma_\mu = 0$) approximately half the time.  As in the
previous example, the heteroskedasticity in the residual variance, together with
the modeling assumption of homoskedasticity, means that the Bayesian and
frequentist covariances are expected to be different.

\SingularResultsGraph{}

We simulated a single dataset (for which the \texttt{lme4} fit was singular),
and computed $\simNumMCMCDraws$ MCMC draws from the model of
\eqref{simple_sim_model} using \texttt{rstanarm}.  With these samples, we
computed the Bayesian posterior covariance and the IJ covariance.  We then
simulated $\simNumSims$ different datasets and ran the same MCMC procedure
for each, computed the posterior mean for each simulation, and computed the
covariance of the posterior means over the simulations.  Ideally, we expect
the IJ covariance to provide a good approximation to the simulation-based
covariance estimate.

The results are show in \figref{simple_sim_result}.  As shown in the left
plot, the posterior covariances of $\log \sigma_y$ and of $\beta$ are
dramatically less than the frequentist variances of $\expect{\post}{\log
\sigma_y}$ and $\expect{\post}{\beta}$.  The posterior of the log
random effect variance, $\log \sigma_\mu$, is extremely non-normal, and
the IJ is not expected to perform well, theoretically.  Nevertheless, we
show that it is a much better approximation to the true frequentist
variance, which is much smaller than the posterior variance.


==> knitr_header.tex <==
\usepackage[]{graphicx}
\usepackage[]{color}
%% maxwidth is the original width if it is less than linewidth
%% otherwise use linewidth (to make sure the graphics do not exceed the margin)
\makeatletter
\def\maxwidth{ %
  \ifdim\Gin@nat@width>\linewidth
    \linewidth
  \else
    \Gin@nat@width
  \fi
}
\makeatother

\definecolor{fgcolor}{rgb}{0.345, 0.345, 0.345}
\newcommand{\hlnum}[1]{\textcolor[rgb]{0.686,0.059,0.569}{#1}}%
\newcommand{\hlstr}[1]{\textcolor[rgb]{0.192,0.494,0.8}{#1}}%
\newcommand{\hlcom}[1]{\textcolor[rgb]{0.678,0.584,0.686}{\textit{#1}}}%
\newcommand{\hlopt}[1]{\textcolor[rgb]{0,0,0}{#1}}%
\newcommand{\hlstd}[1]{\textcolor[rgb]{0.345,0.345,0.345}{#1}}%
\newcommand{\hlkwa}[1]{\textcolor[rgb]{0.161,0.373,0.58}{\textbf{#1}}}%
\newcommand{\hlkwb}[1]{\textcolor[rgb]{0.69,0.353,0.396}{#1}}%
\newcommand{\hlkwc}[1]{\textcolor[rgb]{0.333,0.667,0.333}{#1}}%
\newcommand{\hlkwd}[1]{\textcolor[rgb]{0.737,0.353,0.396}{\textbf{#1}}}%
\let\hlipl\hlkwb

\usepackage{framed}
\makeatletter
\newenvironment{kframe}{%
 \def\at@end@of@kframe{}%
 \ifinner\ifhmode%
  \def\at@end@of@kframe{\end{minipage}}%
  \begin{minipage}{\columnwidth}%
 \fi\fi%
 \def\FrameCommand##1{\hskip\@totalleftmargin \hskip-\fboxsep
 \colorbox{shadecolor}{##1}\hskip-\fboxsep
     % There is no \\@totalrightmargin, so:
     \hskip-\linewidth \hskip-\@totalleftmargin \hskip\columnwidth}%
 \MakeFramed {\advance\hsize-\width
   \@totalleftmargin\z@ \linewidth\hsize
   \@setminipage}}%
 {\par\unskip\endMakeFramed%
 \at@end@of@kframe}
\makeatother

\definecolor{shadecolor}{rgb}{.97, .97, .97}
\definecolor{messagecolor}{rgb}{0, 0, 0}
\definecolor{warningcolor}{rgb}{1, 0, 1}
\definecolor{errorcolor}{rgb}{1, 0, 0}
\newenvironment{knitrout}{}{} % an empty environment to be redefined in TeX

\usepackage{alltt}


==> simple_examples/normal.tex <==
Arguably, the simplest possible misspecified model is a univariate normal
distribution with incorrect variance.  For $\theta \in \mathbb{R}^D$
and $\sigma^2 \ne 1$, let us model our datapoints $\x_n \in \mathbb{R}^D$ as
%
\begin{align*}
%
\textrm{Model:}\quad&&
\theta &\sim \normdist(\cdot | 0, 1)\\
&&x_n &\iid \normdist(\cdot | \theta, 1)\\
\textrm{Data generating process (reality):}\quad&&
\theta &= \thetatrue\\
&&x_n &\iid \normdist(\cdot | \theta, \sigma^2).
%
\end{align*}
%
The model is misspecified because $\sigma^2 \ne 1$.  The posterior mean is
given by
%
\begin{align*}
%
\bar{\x} :={}& \frac{1}{N+1} \sumn \x_n\\
\expect{\post}{\theta} ={}& \bar{\x} \\
\var{\post}{\theta} ={}& \frac{1}{N + 1}\\
\var{\xfdist}{\expect{\post}{\theta}} ={}& \var{\xfdist}{\bar{\x}}
    = \frac{N}{(N+1)^2} \sigma^2.
%
\end{align*}
%
After scaling each by $N$, the posterior variance and frequentist variance
$\var{\xfdist}{\expect{\post}{\theta}}$ do not agree, even asymptotically,
because the model is misspecified.

%
\begin{align*}
%
N \var{\xfdist}{\expect{\post}{\theta}} \plim&
\sigma^2\\
N \var{\post}{\theta} \plim& 1.
%
\end{align*}
%
Let us look at how the sandwich estimator and IJ work in this case. We will take
the function of interest to be $\theta$ itself, so $g(\theta) = \theta$. Here,
the MAP and posterior mean coincide.
%
\begin{align*}
%
\likhat(\x \vert \theta) ={}&
    -\frac{1}{2N} \sumn \left(x_n^2 - 2x_n \theta + \theta^2\right)\\
\log \pi(\theta) ={}& -\frac{1}{2}\theta^2 - \log 2\pi \Rightarrow \\
\thetahat ={}& \bar{\x} \\
\ellgrad{1}(\x \vert \theta) ={}& x_n - \theta\\
\likhatk{2}(\x \vert \theta) ={}& -1.\\
%
\end{align*}
%
Consequently,
%
\begin{align*}
%
\scorecovhat ={}& \meann x_n^2 - \bar{\x}^2 =: \hat\sigma^2 \\
\infohat ={}& 1 \\
\gcovhat ={}& \infohat^{-1} \scorecovhat \infohat^{-1} = \hat\sigma^2.
%
\end{align*}
%
So we see that $\gcovhat$ and $N \var{\xfdist}{\expect{\post}{\theta}}$
coincide asymptotically.

The influence function is as follows.
%
\begin{align*}
%
\infl(\x_n) ={}& N \cov{\post}{
    \theta, -\frac{1}{2} \left(\x_n^2 - 2\x_n \theta + \theta^2 \right)} \\
={}& N \cov{\post}{\theta, \x_n \theta}  + N  \cov{\post}{\theta, \theta^2} \\
={}& \frac{N}{N+1} \x_n + C,
%
\end{align*}
%
where $C$ in the final line is the same for all $\x_n$.  Therefore the
IJ covariance estimate, which is the sample variance of the $\infl(\x_n)$,
is given by
%
\begin{align*}
%
\gcovij ={}& \meann \infl(\x_n)^2 - \bar{\infl}^2 \\
={}& \frac{N^2}{(N + 1)^2} \hat\sigma^2.
%
\end{align*}
%
Thus $\gcovij$ differs from $\gcovhat$ by a factor that vanishes asymptotically,
and $\gcovij$ is also a consistent estimator of the asymptotic
variance $\sigma^2$.

% The bootstrap would draw $\x_n^*$ IID with replacement from the empirical
% distribution on the data points of $\x$.  The bootstrap estimate of the
% $\var{\xfdist}{\expect{\post}{\theta}}$ is the bootstrap estimate of
% $\bar{\x}$, which is also given by $N^2 / (N + 1)^2 \hat\sigma^2$.  In this
% case, the bootstrap and the IJ covariance estimates coincide.


==> simple_examples/poisson.tex <==
Let us now consider another simple non-normal misspecified model, an
over-dispersed Poisson distribution.
%
\begin{align*}
%
\textrm{Model:}\quad&&
\theta &\sim \mathrm{Gamma}(a, b)\\
&&x_n &\iid \mathrm{Poisson}(\theta)\\
\textrm{Data generating process (reality):}\quad&&
\theta &= \thetatrue\\
&&\expect{\xfdist}{x_n} &= \thetatrue \\
&&\var{\xfdist}{x_n} &= \sigma^2 > \thetatrue.
%
\end{align*}
%
The posterior has a closed form:
%
\begin{align*}
%
\bar{\x} :={}& \meann x_n\\
\hat{\sigma}^2 :={}& \meann x_n^2 - \bar{\x}^2\\
\expect{\post}{\theta} ={}& \frac{N\bar{\x} + a}{N + b}\\
\var{\post}{\theta} ={}& \frac{N\bar{\x} + a}{(N + b)^2} \Rightarrow\\
\var{\xfdist}{\expect{\post}{\theta}} ={}& \frac{N \sigma^2}{(N + b)^2}.
%
\end{align*}
%
Because $\x_n$ is over-dispersed, the posterior variance does not match
the frequentist variance $\var{\xfdist}{\expect{\post}{\theta}}$,
even asymptotically.

%
\begin{align*}
%
N \var{\xfdist}{\expect{\post}{\theta}} \plim& \sigma^2\\
N \var{\post}{\theta} \plim& \thetatrue < \sigma^2.
%
\end{align*}
%
The model and MAP are given by
%
\begin{align*}
%
\likhat(\x \vert \theta) ={}&
    \meann \left(x_n \log \theta - \theta \right) + C\\
\log \pi(\theta) ={}& (a - 1) \log \theta - b\theta \Rightarrow \\
\thetahat ={}& \frac{N \bar{\x} + a - 1}{N + b}\\
\ellgrad{1}(\x \vert \theta) ={}& \frac{\x_n}{\theta} - 1 \\
\likhatk{2}(\x \vert \theta) ={}& -\frac{\bar{\x}}{\theta^2}.
%
\end{align*}
%
Here, the MAP and posterior expectation differ by a factor of $1 / (N + b)$,
though, as expected, the difference is $o_p(N^{-1/2})$. We
can now compute the sandwich covariance estimator:
%
\begin{align*}
%
\scorecovhat ={}& \frac{\hat\sigma^2}{\thetahat^{2}} \\
\infohat ={}& -\likhatk{2}(\x \vert \thetahat) = \frac{\bar{\x}}{\thetahat^2}\\
\gcovhat ={}& \infohat^{-1} \scorecovhat \infohat^{-1}
= \frac{\thetahat^2}{\bar{\x}^2} \hat\sigma^2
= \left(\frac{N \bar{\x} + a - 1}{(N + b)\bar{\x}}\right)^2 \hat\sigma^2.
%
\end{align*}
%
As expected, the limits of $N \var{\xfdist}{\expect{\post}{\theta}}$ and
$\gcovhat$ are the same.

The influence function is given by
%
\begin{align*}
%
\infl(\x_n) ={}& N \cov{\post}{\theta, x_n \log \theta - \theta}\\
 ={}& N x_n \cov{\post}{\theta, \log \theta} - N \var{\post}{\theta} \\
 ={}& \frac{N}{N + b} x_n + C.
%
\end{align*}
%
where $C$ is the same for every $\x_n$, and where we have used the posterior
covariance $\cov{\post}{\theta, \log \theta}$ for the Gamma distribution, which
can be found by taking the mixed second-order partial derivative of the log
partition function.  It follows that
%
\begin{align*}
%
\gcovij = \meann \infl(\x_n)^2 - \bar{\infl}^2
    = \frac{N^2}{(N + b)^2} \hat\sigma^2,
%
\end{align*}
%
which is also a consistent estimator of $\sigma^2 = \gcovtrue$.


==> simple_examples/reg_example.tex <==
Before proceeding to a theoretical justifiction of $\gcovij$, let us work out a
simple example, that of linear regression with heteroskedastic noise, analyzed
with model that incorrectly assumes homoskedasticity. Though the posterior for
this problem has a closed form and so does not require MCMC, let alone the IJ
covariance, it will provide an easy-to-understand example of how the IJ
covariance works.

Suppose that we observe regressors, $z_n \in \mathbb{R}^D$, and responses, $y_n
\in \mathbb{R}$, so that our observations are the tuple $\x_n = (z_n, y_n)$.  We
will not specify the data generating process fully, but will assume that the
following laws of large numbers hold:
%
\begin{align*}
%
\hat{M}_{zz} :={}& \meann z_n z_n^T \plim \expect{\xfdist}{z_n z_n^T} =: M_{zz} \\
\hat{M}_{zy} :={}& \meann z_n y_n \plim \expect{\xfdist}{z_n y_n} =: M_{zy}.
%
\end{align*}
%
We additionally assume that $M_{zz}$ is invertible, and that the quantity $z_n
y_n$ obeys a central limit theorem with
%
\begin{align*}
%
V_{zy} :={}& \cov{\xfdist}{z_n y_n}\\
\sqrt{N}\left(\hat{M}_{zy} - M_{zy} \right)
    \dlim& \normdist\left(\cdot \Big\vert 0, V_{zy} \right).
%
\end{align*}

Suppose we use the data to compute a Bayesian posterior using
the following model, with prior parameters $a$, $b$, and $\sigma_\theta$, and
a fixed variance $\sigma$:
%
\begin{align*}
%
\theta &\sim \normdist(\cdot | 0, \sigma_\theta^2 I_D)\\
y_n | \theta, z_n &\indep \normdist(\cdot | \theta^T z_n, \sigma^2).
%
\end{align*}
%
We will take our parameter of interest to be $\theta$ itself, so $g(\theta) =
\theta$.  The posterior has a simple closed form.  Define
%
\begin{align*}
%
\tilde{M}_{zz} :={}& \hat{M}_{zz} + \frac{\sigma_\theta^{-2}}{N} I_D
\quad\quad\textrm{and}\quad\quad
\hat\theta := \tilde{M}_{zz}^{-1} \hat{M}_{zy}.
%
\end{align*}
%
Under these definitions,
$p(\theta \vert \x) =
    \normdist\left(\theta \vert
        \hat\theta,
        N^{-1} \sigma^2 \tilde{M}_{zz}^{-1} \right)$, so
%
\begin{align*}
%
\expect{p(\theta | \x)}{\theta} = \hat\theta
\quad\quad\textrm{and}\quad\quad
N \cov{p(\theta | \x)}{\theta} = \sigma^2 \tilde{M}_{zz}^{-1}
    \plim \sigma^2 M_{zz}^{-1}.
%
\end{align*}
%
It also follows by Slutsky's theorem that $\hat\theta \plim \theta_0 :=
M_{zz}^{-1} M_{zy}$ and
%
\begin{align*}
%
\sqrt{N}\left( \expect{\post}{\theta} - \theta_0 \right)
    \dlim \normdist\left(
            \cdot \Big\vert 0, M_{zz}^{-1} V_{zy} M_{zz}^{-1}
        \right).
%
\end{align*}
%
Thus, $\gcovtrue = M_{zz}^{-1} V_{zy} M_{zz}^{-1}$, and, since $\gcovtrue \ne
\sigma^2 M_{zz}^{-1}$ in general unless the model is correctly specified, the
Bayesian and frequentist limiting covariances do not match in general.

Now let us compute the IJ covariance.  In this case, the log likelihood is
given by
%
\begin{align*}
%
\ell(\x_n \vert \theta) ={}&
    -\frac{1}{2\sigma^2}
        \left(y_n^2 - 2 \theta^T z_n y_n + \theta^T z_n z_n^T \theta \right).
%
\end{align*}
%
The influence function is thus
%
\begin{align*}
%
\infl(\x_n) ={}&
    N \cov{\post}{\theta,
    -\frac{1}{2\sigma^2}\left(y_n^2 - 2 \theta^T z_n y_n +
                             \theta^T z_n z_n^T \theta \right)} \\
={}& N \sigma^{-2} \cov{\post}{\theta} z_n y_n -
\frac{N \sigma^{-2} }{2} \cov{\post}{\theta, \theta^T z_n z_n^T \theta}.
%
\end{align*}
%
To evaluate the second covariance in the preceding display, observe that, for
each $i,j,k$, by normality,
%
\begin{align*}
%
\expect{\post}{
    (\theta_i - \hat\theta_i)
    (\theta_j - \hat\theta_j)
    (\theta_k - \hat\theta_k)} = 0,
%
\end{align*}
%
and that
%
\begin{align*}
%
(\theta - \hat\theta)^T z_n z_n^T (\theta - \hat\theta) ={}&
    \theta^T z_n z_n^T \theta -
    2 \theta^T z_n z_n^T \hat\theta +
    \hat\theta^T z_n z_n^T \hat\theta.
%
\end{align*}
%
Plugging in for $\theta^T z_n z_n^T \theta$ gives
%
\begin{align*}
%
\MoveEqLeft
\cov{\post}{\theta, \theta^T z_n z_n^T \theta} \\
={}& \cov{\post}{\theta, (\theta - \hat\theta)^T z_n z_n^T (\theta - \hat\theta)} +
2 \cov{\post}{\theta, \theta^T z_n z_n^T \hat\theta} -
\cov{\post}{\theta, \hat\theta^T z_n z_n^T \hat\theta} \\ ={}&
2 \cov{\post}{\theta} z_n z_n^T \hat\theta.
%
\end{align*}
%
Combining,
%
\begin{align*}
%
\infl(\x_n) ={}&
    N \sigma^{-2} \cov{\post}{\theta} z_n \left(y_n - z_n^T \hat\theta \right)\\
={}& \tilde{M}_{zz}^{-1} z_n (y_n - z_n^T \hat\theta).
%
\end{align*}
%
We can recognize $\infl(\x_n)$ is very nearly the empirical influence function
of ordinary linear regression.  The only difference is that $\hat\theta$ and
$\tilde{M}_{zz}$ contain a contribution from the prior which vanishes
as $N \rightarrow \infty$.

In particular,
%
\begin{align*}
%
\meann \infl(\x_n) ={}&
    \tilde{M}_{zz}^{-1}
    (\hat{M}_{zy} - \hat{M}_{zz} \tilde{M}_{zz}^{-1} \hat{M}_{zy}) \plim 0\\
\meann \infl(\x_n) \infl(\x_n)^T ={}&
    \tilde{M}_{zz}^{-1}
    \left(\meann z_n z_n^T (y_n - z_n^T \hat\theta)^2\right)
    \tilde{M}_{zz}^{-1}
%
\end{align*}
%
TODO: finish this up, or maybe replace with something simpler.

%


==> simple_examples/regression.tex <==
We now consider multivariate regression with unknown variance.  This will
provide a simple multivariate example, draw a connection with robust frequentist
estimators, and allow us to discuss a point about conditioning on part of
the exchangeable unit.

The model and data generating process are
%
\begin{align*}
%
\textrm{Model:}\quad
&&\sigma^{-2} &\sim \mathrm{Gamma}(a, b)\\
&&\beta &\sim \normdist(\cdot | 0, \sigma_\beta^2 I_D)\\
&&y_n &\iid \normdist(\cdot | \beta^T z_n, \sigma^2)\\
\textrm{Data generating process (reality):}\quad
&&&\textrm{The moments of }
    y_n z_n \textrm{, } z_n z_n^T \textrm{, and } y_n^2 z_n z_n^T\\
&&&\textrm{are finite and obey a LLN, with}\\
&&&\textrm{invertible }\expect{\xfdist}{z_n z_n^T}.
%
\end{align*}
%
Here, $\theta = (\beta, \sigma)$ and $\x_n = (y_n, z_n)$.  We will consider
$g(\theta) = \beta$.  The full posterior has a closed form, but we will only
require the conditional posterior $p(\beta \vert \x, \sigma)$.
%
\begin{align*}
%
\hat{S}_z :={}& \meann z_n z_n^T + \frac{\sigma_\beta^2}{N} I_D\\
\hat\beta :={}& \hat{S}_z^{-1} \left(\meann z_n y_n\right)\\
p(\beta \vert \x, \sigma) ={}&
    \normdist\left(\beta \vert \hat\beta, \sigma^2 \hat{S}_z \right)\\
\expect{\post}{\beta} ={}& \hat\beta\\
\cov{\post}{\beta} ={}& \frac{\sigma^2}{N} \hat{S}_z^{-1}.
%
\end{align*}

In order to consider the frequentist variance of $\expect{\post}{\beta}$, we
have to specify what is random.  Since $\x_n = (z_n, y_n)$, the analysis of
this paper appears to require that both $z_n$ and $y_n$ are random. However, the
generative process for the regressors $z_n$ are not part of the Bayesian model
given above.  Indeed, the generating process for the regressors is hardly
ever specified in Bayesian regression because the data generating
process for $z_n$ is ancillary to the parameters of interest, $\theta$.
However, precisely because $p(z_n)$ is ancillary for $\theta$, one could resolve
this apparent inconsistency by imagining including any data generating process
$p(z_n)$ to the Bayesian model, and observing that the Bayesian posterior is
unchanged no matter what $p(z_n)$ is.

Asymptotically, the difference between random $z_n$ and fixed $z_n$ does not
matter since sample moments over $z_n$ converge to their population
counterparts.  However, in finite sample, the difference can be important, and
it is easier to bootstrap pairs $(z_n, y_n)$ than keep $z_n$ fixed and resample
only $y_n$.  (We will not consider methods such as the residual bootstrap here.)
Unless otherwise stated, we will thus take the view in the present paper that
the full exchangeable pair is random.

Because of the term $\hat{S}_z^{-1}$ and the randomness of $z_n$, the variance
$N \var{\xfdist}{\expect{\post}{\beta}}$ does not have a closed form. However,
by a CLT applied to $\sqrt{N} \meann z_n (y_n - \hat\beta^T z_n)$ and Slutsky's
theorem, the variance is consistently estimated by
%
\begin{align}
%
\hat\epsilon_n :={}& y_n - \hat\beta^T z_n \nonumber\\
N \var{\xfdist}{\expect{\post}{\beta}} \approx&
    \hat{S}_z^{-1} \left(
        \meann \hat\epsilon_n^2 z_n z_n^T \right)
    \hat{S}_z^{-1}.
    \eqlabel{regression_robust_cov}
%
\end{align}
%
If the model is correctly specified, and $\sigma = \sigma_0$, then
%
\begin{align*}
%
\meann z_n z_n^T \hat\epsilon_n^2 \plim \sigma_0^2 \expect{\xfdist}{z_n z_n^T},
%
\end{align*}
%
and $N \var{\xfdist}{\expect{\post}{\beta}}$ coincides asymptotically with
$N \cov{\post}{\beta}$.  However, if the residuals $\hat\epsilon_n$
or their variances are correlated with $z_n$, then the frequentist and Bayesian
covariance will not match, even asymptotically.  The covariance estimate in
\eqref{regression_robust_cov} is known in the frequentist regression literature
as a ``robust'' covariance estimate, and it is sometimes recommended when
there is concern about model misspecification (e.g. \cite[Section
5.5]{davidson:2004:econometric}).  In the present context, it is simply the
regression version of the sandwich covariance matrix $\gcovtrue$.

The influence function in this case is given by
%
\begin{align*}
%
\infl(\x_n) ={}&
    N \cov{\post}{\beta,
    -\frac{1}{2\sigma^2}\left(y_n^2 - 2 \beta^T z_n y_n +
                             \beta^T z_n z_n^T \beta \right)} \\
={}& N \cov{\post}{\beta, \sigma^{-2} \beta} z_n y_n -
\frac{N}{2} \cov{\post}{\beta, \sigma^{-2}} y_n^2 +
\frac{N}{2} \cov{\post}{\beta, \sigma^{-2} \beta^T z_n z_n^T \beta}.
%
\end{align*}
%
First,
%
\begin{align*}
%
\cov{\post}{\beta, \sigma^{-2} \beta} ={}&
\expect{\post}{
    \left(\beta - \hat\beta \right)
    \left(\sigma^{-2} \beta - \expect{\post}{\sigma^{-2} \beta}\right)}
\\ ={}&
\expect{\post}{\left(\beta - \hat\beta \right) \sigma^{-2} \beta}
\\ ={}&
\expect{\post}{
    \sigma^{-2}
    \expect{p(\beta \vert \x, \sigma)}{\left(\beta - \hat\beta \right) \beta}
    }
\\ ={}&
\frac{1}{N} \expect{\post}{\sigma^{-2} \sigma^2 \hat{S}_z^{-1}}
\\ ={}& \frac{1}{N} \hat{S}_z^{-1}.
%
\end{align*}
%
Now, the posterior mean $\expect{\post}{\beta} = \hat\beta$ does not depend on
$\sigma$, so
%
\begin{align*}
%
\cov{\post}{\beta, \sigma^{-2}} ={}&
\expect{\post}{\left(\beta - \hat\beta\right)
               \left( \sigma^{-2} - \expect{\post}{\sigma^{-2}}\right)} \\
={}&
\expect{\post}{\expect{p(\beta \vert \x, \sigma)}{\beta - \hat\beta}
               \left( \sigma^{-2} - \expect{\post}{\sigma^{-2}}\right)} \\
={}& 0.
%
\end{align*}
%
Similarly, the third-order array of third-order covariances is identically zero:
%
\begin{align*}
%
\expect{\post}{\sigma^{-2}(
    \beta - \hat\beta)(\beta - \hat\beta)(\beta - \hat\beta)}
= 0.
%
\end{align*}
%
To use this in $\infl(\x_n)$, observe that
%
\begin{align*}
%
\beta^T z_n z_n^T \beta ={}&
    \left(\beta - \hat\beta\right)^T z_n z_n^T \left(\beta - \hat\beta\right) +
    2 \hat\beta^T z_n z_n^T \beta -
    \hat\beta^T z_n z_n^T \hat\beta,
%
\end{align*}
%
so that
%
\begin{align*}
%
\frac{N}{2} \cov{\post}{\beta, \sigma^{-2} \beta^T z_n z_n^T \beta} ={}&
N \cov{\post}{\beta, \sigma^{-2} \hat\beta^T z_n z_n^T \beta}
\\={}&
N \cov{\post}{\beta, \sigma^{-2} \beta} z_n z_n^T \hat\beta
\\={}&
\hat{S}_z^{-1} z_n z_n^T \hat\beta.
%
\end{align*}
%

%
%
Combining,
%
\begin{align*}
%
\infl(\x_n) = \hat{S}_z^{-1} z_n \left(y_n - z_n^T \hat\beta\right).
%
\end{align*}
%
We thus see that
%
\begin{align*}
%
\bar{\iota} ={}& \hat{S}_z^{-1} \meann z_n y_n = 0\\
\gcovij ={}&
\meann \left(\iota(\x_n)^2 -  \bar{\iota}^2 \right) =
    \hat{S}_z^{-1} \left(
        \meann \hat\epsilon_n^2 z_n z_n^T \right)
    \hat{S}_z^{-1},
%
\end{align*}
%
which matches the frequentist covariance estimate given in
\eqref{regression_robust_cov}.


==> theory_discussion.tex <==

% In this section, we briefly compare our results to selected previous literature
% on the BCLT.

% Standard BCLTs which approximate the posterior are not actaully so different
A standard approach to BCLTs emphasizes the large-data distributional limit of
the Bayesian posterior, e.g., by showing that the total variation distance
between the Bayesian posterior and a normal approximation convergences to zero
in probability.  For example, this is the approach taken by \cite[Chapter
10]{van:2000:asymptotic}, Theorem 1.4.2 of \cite{ghosh:2003:bayesian}, and
\cite{lehman:1983:pointestimation}, on which our proof is principally based.
Results such as our \thmref{bayes_clt_main}, which emphasize the frequentist
properties of posterior quantities, may seem to be of a different character than
distributional approximations to the posterior itself.  However, the approach to
proving convergence in total variation is essentially to prove that posterior
expectations of bounded functions converge uniformly.  Though our assumption of
the differentiability $\psi(\theta, \xvec)$ proscribes the direct use of our
$\thmref{bayes_clt_main}$ to prove convergence in total variation distance, the proof
technique is the same, differing only in whether $\psi(\theta, \xvec)$ is Taylor
expanded in $\theta$ near $\thetahat$.  Indeed, one might argue that many BCLTs
consist of two distinct components: first, to show that only a vanishing ball
around $\thetahat$ matters for the posterior, and, second, to exploit
local properties of the posterior near $\thetahat$ to prove whatever result
is desired.  The first step is, in a sense, generic, and extra assumptions
can be made (or not) in a region of $\thetahat$ to achieve the desired
theoretical aim.  For example, total variation distance forgoes the
expansion of $\psi(\theta, \xvec)$, and a version of our \thmref{bayes_clt_main}
expanding to higher orders requires nothing more than gather the next order
terms in a the local Taylor expansion of posterior quantities.

% We consider data dependence and misspecification
Our \thmref{bayes_clt_main} is distinguished from previous results primarily by
tracking the data dependence; the authors are unaware of any other work that
does so.  Additionally, few previous BCLT results apply under model
misspecification, though \cite{kleijn:2006:misspecification} is a notable
exception.  For example, a result similar to \thmref{bayes_clt_main} is established
by \cite{kass:1990:posteriorexpansions} under stricter differentiability
conditions and for functions $\psi(\theta, \xvec)$ that do not depend on $\xvec$.
Again, however, we emphasize that the proof under misspecification is little
different from the proof under correct specification, just as the proof of the
FCLT (e.g. our \propref{freq_clt}) require little modification to accommodate
misspecification.

% The global uniqueness is a little weird.
As mentioned above, half of a proof of a BCLT typically involves proving that
the behavior of the posterior far from $\thetahat$ is negligible.  To this end,
some assumptions must be made to ensure that the posterior is well behaved
outside a ball centered at $\thetahat$.  For example, one must ensure that there
are no other posterior modes very nearly as high as that at $\thetahat$.  In the
present work we follow \cite{ghosh:2003:bayesian, lehman:1983:pointestimation}
and manage the posterior far from $\thetahat$ with the final condition of
\assuref{bayes_clt}, namely that $\thetatrue$ is a strict optimum of the
empirical likelihood with probability approaching one.  This assumption may seem
somewhat artificial, since it is stated in terms of the data, rather than of any
limiting population quantities.  Recent authors, notably
\cite{kleijn:2006:misspecification}, express a similar requirement in terms of
the existence of a consistent test for $\theta = \thetatrue$, which is more
general and arguably cleaner, but introduces extra complications and  perhaps
obscure somewhat the role of the assumption in the proof.  Suffice to say, the
uniqueness of the optimum in misspecified BCLTs is a serious issue, but a
complicated one that is beyond the scope of the present paper, and we
essentially assume the problem away.  Again, see
\cite{kleijn:2006:misspecification} for a more thorough discussion.


==> what_is_random.tex <==

What does it mean in the context of this model to consider the data to be IID?
This question is inseparable from what we consider to be a datapoint, $\x_n$.
There are several reasonable answers to this question, corresponding to
different sorts of notions of ``drawing a new sample.'' We will show that, by
assuming that the functions $\ell(\x_n \vert \gamma, \lambda)$ are IID (as in
\secref{basics}), the frequentist variability we study corresponds to assuming
that the random effects are fixed, were we to believe in the model.

First, note that $\ell(\x_n \vert \gamma, \lambda)$ cannot be identically
distributed if the regressors and random effect indices are fixed.  A unit of
data must then consist of the tuple $\x_n = (\y_n, \r_n, \a_n)$, and when we
model $\x_n \iid \fdist$, we mean that the regressors, random effect index, and
response are all IID random.

Modeling $(\y_n, \r_n, \a_n) \iid \fdist$ in this way is a completely
non-parametric assumption, but we can ask what it means in the context of our
assumed model.  First, note that the distribution of $\a$ and $\r$ are not
posited to depend on $\theta$ in any way, so their distributions do not affect
the posterior.  However, the fact that $\a_n$ is included in the definition of a
datapoint implies that we are conditioning on the random effects $\lambda$,
since we assume that two distinct data points $n$ and $m$ that have been
assigned to the same random effect (i.e. $\a_n = \a_m$) are independent of one
another.  Call IID draws of $\x_n = (\y_n, \r_n, \a_n)$ the ``conditional
distribution.''

In the context of our toy problem, drawing from the conditional distribution
would correspond to the question: How variable would our posterior expectation
be if we performed new observations at the same sites as the original analysis?
We emphasize that, in many applications, including those in \secref{experiments}
below, this is a very reasonable question to ask.

One might instead (or additionally) be interested in a different IID
distribution, which is the distribution of a datapoint $\x_n' = (\y_n, \r_n)$,
marginally over the random effects.  Call this the ``marginal distribution.'' Of
course, for $\x_n'$ to be IID, one would require each observation to be
associated with exactly one distinct random effect, with $G = N$ and $\a_n \ne
\a_m$ for $n \ne m$.  Under this assumption, the $\a_n$ cannot be independently
distributed.

In the context of our toy problem, drawing from the marginal distribution would
correspond to the question: How variable would our posterior expectation be if
we performed new observations at a new set of sites?
%
Both the marginal and conditional distribution may be practically interesting,
depending on the context.  But the conditional question is easier to answer
computationally from MCMC samples when the marginal likelihood is intractable.
Formally, the marginal question involves re-sampling the functions
%
\begin{align*}
%
\ell(\x_n' | \gamma) =
    \log \int \exp(\ell(\x_n' \vert \gamma, \lambda_n))
        \p(\lambda_n \vert \gamma)
    d\lambda.
%
\end{align*}
%
Though this marginal distribution is tractable our toy example, one typically
turns to MCMC precisely because one cannot analytically marginalize over the
random effect, i.e., one cannot compute the function $\ell(\x_n' \vert \gamma)$.
In contrast, the IJ covariance based on $\ell(\x_n \vert \gamma, \lambda)$ is
tractable, but can only estimate the conditional variance, not the marginal
variance.

Furthermore, in many cases, the random effects are not fully nested, so it is
not possible to partition the observations so that each partition depends on a
disjoint set of $\lambda$ parameters (we give a real-life example in
\secref{arm_pilots} below).  In such cases there is no natural way to express a
marginal IID distribution over datapoints.  However, the conditional IID
assumption still makes sense, as long as the indices mapping a datapoint to the
random effects are also considered random.

A potentially confusing case occurs when, in the original dataset, each
observation has its own single random effect, so that $G=N$ and $\a_n = n$.
In this case, the posterior expectation $\expect{\post}{\g(\theta)}$ is
identical as a function of $\xvec$ whether one uses the marginal log likelihood
$\ell(\y_n \vert \gamma)$ or conditional log likelihood $\ell(\y_n \vert \gamma,
\lambda_n)$ in the model.  Given this, one might wonder how one could possible
represent conditional versus marginal sampling nonparametrically.  The answer is
that under conditional sampling a particular random effects $\lambda_n$ may
occur multiple times (or not at all) under sampling from $\fdist$, whereas,
under marginal sampling, each random effect occurs precisely once in the
posterior.\footnote{Given that $\a_n = n$ is an extremely unlikely draw
under conditional sampling, one might argue that conditional sampling is an
unrealistic model for such a dataset, and that the data is better modeled as
exchangeable than IID. How to estimate the frequentist variance
nonparametrically under non-IID exchangeability is an important question but
beyond the scope of the present work.}

The bootstrap as described in \algrref{boot} embeds the difference between
conditional and marginal sampling in a subtle way.  For example, in our toy
model, suppose that the $n$-th datapoint is chosen to occur twice in the
bootstrap sample $\xvec^*$. Do the two contributions to the posterior $\p(\theta
\vert \xvec^*)$ depend on the same $\lambda_{\a_n}$, or does each get its
own, distinct random effect, ignoring the fact that the two bootstrapped data
points came from the same original data point?  These choices correspond to the
conditional and marginal variances, respectively.  In this way, the bootstrap
is able to estimate both conditional and marginal frequentist variances,
though at the cost of using MCMC to marginalize over $\lambda$ for each
bootstrap sample.

